Safe Reinforcement Learning via Shielding under Partial Observability

Safe exploration is a common problem in reinforcement learning (RL) that aims to prevent agents from making disastrous decisions while exploring their environment. A family of approaches to this problem assume domain knowledge in the form of a (partial) model of this environment to decide upon the safety of an action. A so-called shield forces the RL agent to select only safe actions. However, for adoption in various applications, one must look beyond enforcing safety and also ensure the applicability of RL with good performance. We extend the applicability of shields via tight integration with state-of-the-art deep RL, and provide an extensive, empirical study in challenging, sparse-reward environments under partial observability. We show that a carefully integrated shield ensures safety and can improve the convergence rate and final performance of RL agents. We furthermore show that a shield can be used to bootstrap state-of-the-art RL agents: they remain safe after initial learning in a shielded setting, allowing us to disable a potentially too conservative shield eventually.

==> compute_times.tex <==
\begin{table}[h!]
	\centering
%	\raisebox{0pt}[\dimexpr\height-3\baselineskip\relax]{
		\scalebox{1.0}{
%			\scriptsize\setlength{\tabcolsep}{3.5pt}
			\begin{tabular}{@{}L{4cm}R{1cm}R{1cm}R{1cm}R{1cm}@{}}
				\toprule
				Domain & Constants & $|S|$ & $|\Act|$ & $|\ObsSym|$\\
				\midrule
				\domain{Rocks}  & & & &  \\
				\domain{Rocks}  & & & &  \\
				\domain{Rocks}  & & & &  \\
				\domain{Rocks}  & & & &  \\
				\domain{Rocks}  & & & &  \\
				\domain{Rocks}  & & & &  \\
				\bottomrule
		\end{tabular}}
%	}%
	\captionof{table}{Benchmark metrics (LTL examples in gray) \label{tab:example_metrics}.}	
\end{table}

==> figs/data/Ablation/obstacle_full_obs_noshield.tex <==
\pgfplotstableread{
0.000000000000000000e+00 -0.99e+02 -9.900000000000000000e+02 9.910000000000000000e+02 9.896950073242187500e+02 9.917050170898437500e+02 9.905279722285947628e+02 9.908720521854677372e+02
1.000000000000000000e+02 -0.99e+02  9.900000000000000000e+02 9.911443000000000438e+02 9.898560180664062500e+02 9.919440307617187500e+02 9.907279844356260128e+02 9.910720643924989872e+02
2.000000000000000000e+02 9.910000000000000000e+02 9.900000000000000000e+02 9.920000000000000000e+02 9.899045410156250000e+02 9.920954589843750000e+02 9.908279600215635128e+02 9.911720399784364872e+02
3.000000000000000000e+02 9.912000122070312500e+02 9.910000000000000000e+02 9.920000000000000000e+02 9.904516601562500000e+02 9.919483642578125000e+02 9.910279722285947628e+02 9.913720521854677372e+02
4.000000000000000000e+02 9.910999755859375000e+02 9.910000000000000000e+02 9.910000000000000000e+02 9.905614624023437500e+02 9.916384887695312500e+02 9.909279356075010128e+02 9.912720155643739872e+02
5.000000000000000000e+02 9.909800048828125227e+02 9.903999999999999773e+02 9.914288599999999860e+02 9.900937377929687955e+02 9.918662719726562500e+02 1.000000000000000000e+01 1.000000000000000000e+01
6.000000000000000000e+02 9.910599975585937500e+02 9.906000000000000227e+02 9.914288599999999860e+02 9.902670288085937500e+02 9.918529663085937500e+02 1.000000000000000000e+01 1.000000000000000000e+01
7.000000000000000000e+02 9.911399902343749773e+02 9.906000000000000227e+02 9.916000000000000227e+02 9.903183349609374773e+02 9.919616455078124773e+02 1.000000000000000000e+01 1.000000000000000000e+01
8.000000000000000000e+02 9.911599853515624545e+02 9.907999999999999545e+02 9.914288599999999860e+02 9.904174194335937500e+02 9.919025512695312727e+02 1.000000000000000000e+01 1.000000000000000000e+01
9.000000000000000000e+02 9.910399780273437500e+02 9.906000000000000227e+02 9.912288599999999406e+02 9.902870849609374773e+02 9.917928710937500227e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.000000000000000000e+03 9.911199829101562955e+02 9.906000000000000227e+02 9.914288599999999860e+02 9.903135498046874545e+02 9.919264160156250227e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.100000000000000000e+03 9.909599853515625227e+02 9.903999999999999773e+02 9.912577199999999493e+02 9.901696044921875455e+02 9.917503662109375000e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.200000000000000000e+03 9.908399902343750227e+02 9.903999999999999773e+02 9.910865799999999126e+02 9.901070922851562273e+02 9.915728881835937045e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.300000000000000000e+03 9.908199951171875455e+02 9.903711399999999685e+02 9.910865799999999126e+02 9.900721801757812273e+02 9.915678100585937500e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.400000000000000000e+03 9.909199951171874545e+02 9.905711400000000140e+02 9.911154399999999214e+02 9.901921752929687273e+02 9.916478149414062955e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.500000000000000000e+03 9.908799926757812955e+02 9.905711400000000140e+02 9.911154399999999214e+02 9.901853515625000455e+02 9.915746337890625455e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.600000000000000000e+03 9.910799926757812273e+02 9.907711400000000594e+02 9.914865800000000036e+02 9.902969970703125000e+02 9.918629882812499545e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.700000000000000000e+03 9.910199951171874773e+02 9.907711400000000594e+02 9.914577199999999948e+02 9.903190307617187500e+02 9.917209594726562045e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.800000000000000000e+03 9.910799926757812273e+02 9.907999999999999545e+02 9.916288600000000315e+02 9.904058837890625000e+02 9.917541015624999545e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.900000000000000000e+03 9.910599975585937500e+02 9.906000000000000227e+02 9.917999999999999545e+02 9.903470092773437727e+02 9.917729858398437273e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.000000000000000000e+03 9.909599975585937273e+02 9.903999999999999773e+02 9.916000000000000227e+02 9.901791137695312273e+02 9.917408813476562273e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.100000000000000000e+03 9.908800048828125000e+02 9.902000000000000455e+02 9.913999999999999773e+02 9.900904418945312955e+02 9.916695678710937045e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.200000000000000000e+03 9.910199951171874773e+02 9.902000000000000455e+02 9.916000000000000227e+02 9.901397216796874545e+02 9.919002685546875000e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.300000000000000000e+03 9.909599975585937273e+02 9.902000000000000455e+02 9.913999999999999773e+02 9.900812988281250000e+02 9.918386962890624545e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.400000000000000000e+03 9.910000000000000000e+02 9.903711399999999685e+02 9.913999999999999773e+02 9.901042236328124773e+02 9.918957763671875227e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.500000000000000000e+03 9.910000000000000000e+02 9.905422800000000052e+02 9.913999999999999773e+02 9.901801879882812045e+02 9.918198120117187955e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.600000000000000000e+03 9.910399902343749545e+02 9.907134200000000419e+02 9.914288599999999860e+02 9.902201782226562727e+02 9.918598022460937500e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.700000000000000000e+03 9.909799926757812045e+02 9.907134200000000419e+02 9.912577199999999493e+02 9.901745117187499545e+02 9.917854736328124545e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.800000000000000000e+03 9.909999877929687955e+02 9.905134199999999964e+02 9.914577199999999948e+02 9.901121948242187045e+02 9.918877807617187727e+02 1.000000000000000000e+01 1.000000000000000000e+01
2.900000000000000000e+03 9.909999877929687955e+02 9.905134199999999964e+02 9.914577199999999948e+02 9.901121948242187045e+02 9.918877807617187727e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.000000000000000000e+03 9.909999877929687955e+02 9.903422800000000734e+02 9.914865800000000036e+02 9.900578369140624773e+02 9.919421386718750000e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.100000000000000000e+03 9.910399902343749545e+02 9.903422800000000734e+02 9.916577199999999266e+02 9.901065185546874545e+02 9.919734619140624545e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.200000000000000000e+03 9.910799926757812273e+02 9.905134199999999964e+02 9.916577199999999266e+02 9.901659545898437500e+02 9.919940307617187045e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.300000000000000000e+03 9.910799926757812273e+02 9.906845600000000331e+02 9.916577199999999266e+02 9.902086181640625000e+02 9.919513671874999545e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.400000000000000000e+03 9.910999877929687045e+02 9.906845600000000331e+02 9.916577199999999266e+02 9.902445678710937500e+02 9.919554077148437727e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.500000000000000000e+03 9.911199951171875000e+02 9.906845600000000331e+02 9.916288600000000315e+02 9.902117675781249773e+02 9.920282226562500227e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.600000000000000000e+03 9.909199951171874545e+02 9.905134199999999964e+02 9.912577199999999493e+02 9.901001220703125227e+02 9.917398681640625000e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.700000000000000000e+03 9.910000000000000000e+02 9.905422800000000052e+02 9.914288599999999860e+02 9.901310913085937955e+02 9.918689086914062045e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.800000000000000000e+03 9.908999999999999773e+02 9.903711399999999685e+02 9.912288599999999406e+02 9.900372314453125000e+02 9.917627685546874545e+02 1.000000000000000000e+01 1.000000000000000000e+01
3.900000000000000000e+03 9.907599975585937955e+02 9.902000000000000455e+02 9.910288600000000088e+02 9.899792602539062045e+02 9.915407348632812727e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.000000000000000000e+03 9.906999877929687273e+02 9.902000000000000455e+02 9.910288600000000088e+02 9.900137451171874545e+02 9.913862304687500000e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.100000000000000000e+03 9.909199951171874545e+02 9.903999999999999773e+02 9.913999999999999773e+02 9.901654052734375000e+02 9.916745849609375227e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.200000000000000000e+03 9.906999877929687273e+02 9.902000000000000455e+02 9.910288600000000088e+02 9.900577026367187727e+02 9.913422729492187955e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.300000000000000000e+03 9.908199951171875455e+02 9.903999999999999773e+02 9.910577200000000175e+02 9.901633544921875227e+02 9.914766357421874545e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.400000000000000000e+03 9.910000000000000000e+02 9.906000000000000227e+02 9.912577199999999493e+02 9.903071655273437273e+02 9.916928344726562727e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.500000000000000000e+03 9.910400024414062727e+02 9.906000000000000227e+02 9.912577199999999493e+02 9.903301635742187727e+02 9.917498413085937727e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.600000000000000000e+03 9.910799926757812273e+02 9.906000000000000227e+02 9.912577199999999493e+02 9.903974853515625227e+02 9.917625000000000455e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.700000000000000000e+03 9.912000000000000455e+02 9.907711400000000594e+02 9.914288599999999860e+02 9.904691406250000227e+02 9.919308593749999545e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.800000000000000000e+03 9.912000000000000455e+02 9.907422800000000507e+02 9.916000000000000227e+02 9.904691406250000227e+02 9.919308593749999545e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.900000000000000000e+03 9.910400024414062727e+02 9.905422800000000052e+02 9.913999999999999773e+02 9.903152465820312500e+02 9.917647583007812955e+02 1.000000000000000000e+01 1.000000000000000000e+01
5.000000000000000000e+03 9.910600097656249545e+02 9.905422800000000052e+02 9.914288599999999860e+02 9.903187866210937500e+02 9.918012329101562727e+02 1.000000000000000000e+01 1.000000000000000000e+01
}\obstacleFullObsNoShield


==> figs/data/Ablation/obstacle_full_obs_shield.tex <==
\pgfplotstableread{
0.000000000000000000e+00 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -5.349700121141285081e+02 3.369700121141285081e+02
1.000000000000000000e+02 9.909000244140625000e+02 9.900000000000000000e+02 9.911443000000000438e+02 9.900693359375000000e+02 9.917307128906250000e+02 5.549300122999339919e+02 1.426870036528191122e+03
2.000000000000000000e+02 9.910999755859375000e+02 9.900000000000000000e+02 9.920000000000000000e+02 9.901565551757812500e+02 9.920433959960937500e+02 5.551299634718089919e+02 1.427069987700066122e+03
3.000000000000000000e+02 9.909000244140625000e+02 9.910000000000000000e+02 9.910000000000000000e+02 9.903615112304687500e+02 9.914385375976562500e+02 5.549300122999339919e+02 1.426870036528191122e+03
4.000000000000000000e+02 9.907999877929687500e+02 9.900000000000000000e+02 9.911443000000000438e+02 9.899282226562500000e+02 9.916717529296875000e+02 5.548299756788402419e+02 1.426769999907097372e+03
5.000000000000000000e+02 7.729400024414062500e+02 7.723999999999999773e+02 7.732577199999999493e+02 7.723031250000000227e+02 7.735768798828124773e+02 0.000000000000000000e+00 1.000000000000000000e+01
6.000000000000000000e+02 9.909200073242187727e+02 9.902000000000000455e+02 9.912577199999999493e+02 9.900944458007812727e+02 9.917455688476562727e+02 1.000000000000000000e+01 1.000000000000000000e+01
7.000000000000000000e+02 9.910000000000000000e+02 9.903999999999999773e+02 9.914288599999999860e+02 9.901843750000000455e+02 9.918156249999999545e+02 1.000000000000000000e+01 1.000000000000000000e+01
8.000000000000000000e+02 9.911000000000000227e+02 9.906000000000000227e+02 9.914288599999999860e+02 9.903130615234374545e+02 9.918869384765624773e+02 1.000000000000000000e+01 1.000000000000000000e+01
9.000000000000000000e+02 9.911799926757812500e+02 9.906000000000000227e+02 9.914577199999999948e+02 9.903445556640624545e+02 9.920154296875000455e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.000000000000000000e+03 9.912599975585937955e+02 9.907711400000000594e+02 9.916288600000000315e+02 9.904029541015625000e+02 9.921170410156249773e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.100000000000000000e+03 9.913199951171875455e+02 9.907711400000000594e+02 9.918288599999999633e+02 9.904183959960937500e+02 9.922215942382812273e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.200000000000000000e+03 9.913199951171875455e+02 9.905711400000000140e+02 9.918288599999999633e+02 9.903371093749999545e+02 9.923028808593750227e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.300000000000000000e+03 9.913199951171875455e+02 9.907134200000000419e+02 9.918288599999999633e+02 9.902744018554687955e+02 9.923655883789062955e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.400000000000000000e+03 9.911799926757812500e+02 9.905134199999999964e+02 9.917999999999999545e+02 9.901306030273437955e+02 9.922293823242187045e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.500000000000000000e+03 9.910999877929687045e+02 9.903422800000000734e+02 9.916288600000000315e+02 9.900722045898437500e+02 9.921277709960937727e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.600000000000000000e+03 9.910199829101562727e+02 9.903422800000000734e+02 9.914288599999999860e+02 9.900757690429687727e+02 9.919641967773437727e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.700000000000000000e+03 9.908799804687499773e+02 9.903422800000000734e+02 9.912288599999999406e+02 9.900132568359374545e+02 9.917467041015625000e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.800000000000000000e+03 9.907199829101562045e+02 9.900000000000000000e+02 9.910288600000000088e+02 9.898800048828125000e+02 9.915599609375000227e+02 1.000000000000000000e+01 1.000000000000000000e+01
1.900000000000000000e+03 7.727999877929687500e+02 7.722000000000000455e+02 7.730288600000000088e+02 7.721200073242187045e+02 7.734799682617187955e+02 0.000000000000000000e+00 1.000000000000000000e+01
2.000000000000000000e+03 5.548399902343750227e+02 5.543999999999999773e+02 5.550000000000000000e+02 5.543343627929687045e+02 5.553456176757812273e+02 0.000000000000000000e+00 1.000000000000000000e+01
2.100000000000000000e+03 5.549599975585937273e+02 5.545711400000000140e+02 5.552000000000000455e+02 5.544000854492187500e+02 5.555199096679687045e+02 0.000000000000000000e+00 1.000000000000000000e+01
2.200000000000000000e+03 5.550000000000000000e+02 5.545711400000000140e+02 5.552000000000000455e+02 5.544504150390624773e+02 5.555495849609375227e+02 0.000000000000000000e+00 1.000000000000000000e+01
2.300000000000000000e+03 3.370400024414062727e+02 3.367711400000000026e+02 3.371999999999999886e+02 3.366863769531249773e+02 3.373936279296875114e+02 0.000000000000000000e+00 1.000000000000000000e+01
2.400000000000000000e+03 3.370400024414062727e+02 3.367711400000000026e+02 3.371999999999999886e+02 3.366863769531249773e+02 3.373936279296875114e+02 0.000000000000000000e+00 1.000000000000000000e+01
2.500000000000000000e+03 3.370400024414062727e+02 3.367711400000000026e+02 3.371999999999999886e+02 3.366863769531249773e+02 3.373936279296875114e+02 0.000000000000000000e+00 1.000000000000000000e+01
2.600000000000000000e+03 1.189599975585937557e+02 1.187999999999999972e+02 1.190000000000000000e+02 1.188103271484374943e+02 1.191096679687500028e+02 0.000000000000000000e+00 1.000000000000000000e+01
2.700000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
2.800000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
2.900000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.000000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.100000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.200000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.300000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.400000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.500000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.600000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.700000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.800000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
3.900000000000000000e+03 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 -9.900000000000000000e+01 0.000000000000000000e+00 0.000000000000000000e+00
4.000000000000000000e+03 1.190999999999999943e+02 1.190000000000000000e+02 1.192000000000000028e+02 1.188950561523437557e+02 1.193049438476562472e+02 0.000000000000000000e+00 1.000000000000000000e+01
4.100000000000000000e+03 3.371599975585937727e+02 3.369711399999999912e+02 3.373999999999999773e+02 3.367540527343750227e+02 3.375659423828125227e+02 0.000000000000000000e+00 1.000000000000000000e+01
4.200000000000000000e+03 5.551199951171875000e+02 5.547711400000000594e+02 5.553999999999999773e+02 5.545643798828125455e+02 5.556756103515624545e+02 0.000000000000000000e+00 1.000000000000000000e+01
4.300000000000000000e+03 7.731799926757812500e+02 7.727422800000000507e+02 7.736000000000000227e+02 7.724043823242187727e+02 7.739556030273437273e+02 0.000000000000000000e+00 1.000000000000000000e+01
4.400000000000000000e+03 9.911799926757812500e+02 9.907134200000000419e+02 9.916000000000000227e+02 9.902255004882812273e+02 9.921344848632812727e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.500000000000000000e+03 9.910399902343749545e+02 9.905134199999999964e+02 9.914288599999999860e+02 9.901160888671875000e+02 9.919638916015625227e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.600000000000000000e+03 9.910199951171874773e+02 9.905422800000000052e+02 9.912577199999999493e+02 9.901770996093749773e+02 9.918628906249999773e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.700000000000000000e+03 9.911000000000000227e+02 9.907134200000000419e+02 9.914577199999999948e+02 9.902108154296875000e+02 9.919891845703125455e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.800000000000000000e+03 9.910599975585937500e+02 9.907422800000000507e+02 9.912865799999999581e+02 9.902508056640624545e+02 9.918691894531250455e+02 1.000000000000000000e+01 1.000000000000000000e+01
4.900000000000000000e+03 9.910799926757812273e+02 9.907711400000000594e+02 9.912865799999999581e+02 9.903896850585937273e+02 9.917703002929687273e+02 1.000000000000000000e+01 1.000000000000000000e+01
5.000000000000000000e+03 9.911199951171875000e+02 9.909711399999999912e+02 9.912577199999999493e+02 9.904775512695312045e+02 9.917624389648437955e+02 1.000000000000000000e+01 1.000000000000000000e+01
}\obstacleFullObsShield

==> figs/data/Representations/obstacle.tex <==
\pgfplotstableread{
0.000000000000000000e+00 -1.990000000000000000e+02
1.000000000000000000e+02 9.910000000000000000e+02
2.000000000000000000e+02 9.905999755859375000e+02
3.000000000000000000e+02 9.912000122070312500e+02
4.000000000000000000e+02 9.905999755859375000e+02
5.000000000000000000e+02 9.908399902343750227e+02
6.000000000000000000e+02 9.911599975585937727e+02
7.000000000000000000e+02 9.912000000000000455e+02
8.000000000000000000e+02 9.912800048828124773e+02
9.000000000000000000e+02 9.912800048828124773e+02
1.000000000000000000e+03 9.914000122070312955e+02
1.100000000000000000e+03 9.911600097656249773e+02
1.200000000000000000e+03 9.912000122070312500e+02
1.300000000000000000e+03 9.912000122070312500e+02
1.400000000000000000e+03 9.913200073242187500e+02
1.500000000000000000e+03 9.911200073242187045e+02
1.600000000000000000e+03 9.910400024414062727e+02
1.700000000000000000e+03 9.910400024414062727e+02
1.800000000000000000e+03 9.910400024414062727e+02
1.900000000000000000e+03 9.908800048828125000e+02
2.000000000000000000e+03 9.910000000000000000e+02
2.100000000000000000e+03 9.908800048828125000e+02
2.200000000000000000e+03 9.910000000000000000e+02
2.300000000000000000e+03 9.910800048828125455e+02
2.400000000000000000e+03 9.910800048828125455e+02
2.500000000000000000e+03 9.912000122070312500e+02
2.600000000000000000e+03 9.913600097656250227e+02
2.700000000000000000e+03 9.910000122070312045e+02
2.800000000000000000e+03 9.908800048828125000e+02
2.900000000000000000e+03 9.908400024414062273e+02
3.000000000000000000e+03 9.907199951171875227e+02
3.100000000000000000e+03 9.908399902343750227e+02
3.200000000000000000e+03 9.908799926757812955e+02
3.300000000000000000e+03 9.908799926757812955e+02
3.400000000000000000e+03 9.910000000000000000e+02
3.500000000000000000e+03 9.912400024414062045e+02
3.600000000000000000e+03 9.912000122070312500e+02
3.700000000000000000e+03 9.914400024414062500e+02
3.800000000000000000e+03 9.914800048828125227e+02
3.900000000000000000e+03 9.912400024414062045e+02
4.000000000000000000e+03 9.910000000000000000e+02
4.100000000000000000e+03 9.909199951171874545e+02
4.200000000000000000e+03 9.908800048828125000e+02
4.300000000000000000e+03 9.907999999999999545e+02
4.400000000000000000e+03 9.908400024414062273e+02
4.500000000000000000e+03 9.908800048828125000e+02
4.600000000000000000e+03 9.908800048828125000e+02
4.700000000000000000e+03 9.907599975585937955e+02
4.800000000000000000e+03 9.909599975585937273e+02
4.900000000000000000e+03 9.909999877929687955e+02
5.000000000000000000e+03 9.910799926757812273e+02
}\obstacleshieldREINFORCESupp

\pgfplotstableread{
0.000000000000000000e+00 -1.990000000000000000e+02
1.000000000000000000e+02 -1.990000000000000000e+02
2.000000000000000000e+02 -1.990000000000000000e+02
3.000000000000000000e+02 -1.990000000000000000e+02
4.000000000000000000e+02 -1.990000000000000000e+02
5.000000000000000000e+02 -1.990000000000000000e+02
6.000000000000000000e+02 -1.990000000000000000e+02
7.000000000000000000e+02 -1.990000000000000000e+02
8.000000000000000000e+02 -1.990000000000000000e+02
9.000000000000000000e+02 -1.990000000000000000e+02
1.000000000000000000e+03 -1.990000000000000000e+02
1.100000000000000000e+03 -1.990000000000000000e+02
1.200000000000000000e+03 -1.990000000000000000e+02
1.300000000000000000e+03 -1.990000000000000000e+02
1.400000000000000000e+03 -1.990000000000000000e+02
1.500000000000000000e+03 -1.990000000000000000e+02
1.600000000000000000e+03 -1.990000000000000000e+02
1.700000000000000000e+03 -1.990000000000000000e+02
1.800000000000000000e+03 -1.990000000000000000e+02
1.900000000000000000e+03 3.908000488281250284e+01
2.000000000000000000e+03 2.770800048828124886e+02
2.100000000000000000e+03 5.151200073242187045e+02
2.200000000000000000e+03 7.530400024414062727e+02
2.300000000000000000e+03 9.910800048828125455e+02
2.400000000000000000e+03 9.910000000000000000e+02
2.500000000000000000e+03 9.910400024414062727e+02
2.600000000000000000e+03 9.909199951171874545e+02
2.700000000000000000e+03 9.909199951171874545e+02
2.800000000000000000e+03 9.911199951171875000e+02
2.900000000000000000e+03 9.910000000000000000e+02
3.000000000000000000e+03 9.908400024414062273e+02
3.100000000000000000e+03 9.908000122070312727e+02
3.200000000000000000e+03 9.908800170898437045e+02
3.300000000000000000e+03 9.906800170898437727e+02
3.400000000000000000e+03 9.907600097656250000e+02
3.500000000000000000e+03 9.909600097656250455e+02
3.600000000000000000e+03 9.910400024414062727e+02
3.700000000000000000e+03 9.912000000000000455e+02
3.800000000000000000e+03 9.911599975585937727e+02
3.900000000000000000e+03 9.911599975585937727e+02
4.000000000000000000e+03 9.911199951171875000e+02
4.100000000000000000e+03 9.910799926757812273e+02
4.200000000000000000e+03 9.907599975585937955e+02
4.300000000000000000e+03 9.908400024414062273e+02
4.400000000000000000e+03 9.909600097656250455e+02
4.500000000000000000e+03 9.907600097656250000e+02
4.600000000000000000e+03 9.907600097656250000e+02
4.700000000000000000e+03 9.908000122070312727e+02
4.800000000000000000e+03 9.906000122070312273e+02
4.900000000000000000e+03 9.906800048828124545e+02
5.000000000000000000e+03 9.908400024414062273e+02
}\obstacleshieldREINFORCEObs

\pgfplotstableread{
0.000000000000000000e+00 -3.593999938964843750e+02
1.000000000000000000e+02 -8.417999877929687500e+02
2.000000000000000000e+02 -6.802000122070312500e+02
3.000000000000000000e+02 -1.003000000000000000e+03
4.000000000000000000e+02 -1.002599975585937500e+03
5.000000000000000000e+02 -7.773999938964843750e+02
6.000000000000000000e+02 -8.417999999999999545e+02
7.000000000000000000e+02 -8.419200073242187727e+02
8.000000000000000000e+02 -8.422000000000000455e+02
9.000000000000000000e+02 -8.099199951171874545e+02
1.000000000000000000e+03 -7.777999999999999545e+02
1.100000000000000000e+03 -8.420000000000000000e+02
1.200000000000000000e+03 -8.097599975585937955e+02
1.300000000000000000e+03 -8.739200073242187727e+02
1.400000000000000000e+03 -8.738800170898437045e+02
1.500000000000000000e+03 -9.060400146484374773e+02
1.600000000000000000e+03 -8.738000122070312727e+02
1.700000000000000000e+03 -9.381200073242187045e+02
1.800000000000000000e+03 -9.060400024414062727e+02
1.900000000000000000e+03 -9.061199951171875000e+02
2.000000000000000000e+03 -8.419599975585937273e+02
2.100000000000000000e+03 -8.420799926757812273e+02
2.200000000000000000e+03 -8.420000000000000000e+02
2.300000000000000000e+03 -7.455599975585937500e+02
2.400000000000000000e+03 -7.135599975585937500e+02
2.500000000000000000e+03 -7.456000000000000227e+02
2.600000000000000000e+03 -7.777200073242187273e+02
2.700000000000000000e+03 -7.457200073242187273e+02
2.800000000000000000e+03 -7.457200073242187273e+02
2.900000000000000000e+03 -7.776800048828124545e+02
3.000000000000000000e+03 -8.096000000000000227e+02
3.100000000000000000e+03 -7.453599975585937045e+02
3.200000000000000000e+03 -7.452799926757812727e+02
3.300000000000000000e+03 -8.415199951171874773e+02
3.400000000000000000e+03 -8.094800048828125227e+02
3.500000000000000000e+03 -7.452800048828124773e+02
3.600000000000000000e+03 -6.810400024414062727e+02
3.700000000000000000e+03 -6.166800048828124545e+02
3.800000000000000000e+03 -5.847999999999999545e+02
3.900000000000000000e+03 -5.526799926757812500e+02
4.000000000000000000e+03 -6.167999999999999545e+02
4.100000000000000000e+03 -6.810400024414062727e+02
4.200000000000000000e+03 -6.810400024414062727e+02
4.300000000000000000e+03 -6.809200073242187727e+02
4.400000000000000000e+03 -7.452000122070312500e+02
4.500000000000000000e+03 -7.456400024414062955e+02
4.600000000000000000e+03 -7.134800048828125227e+02
4.700000000000000000e+03 -6.813600036621094205e+02
4.800000000000000000e+03 -7.135200012207030795e+02
4.900000000000000000e+03 -6.813600036621094205e+02
5.000000000000000000e+03 -6.812400085449219205e+02
}\obstaclenoshieldREINFORCESupp

\pgfplotstableread{
0.000000000000000000e+00 -5.202000122070312500e+02
1.000000000000000000e+02 -1.003200012207031250e+03
2.000000000000000000e+02 -6.810000000000000000e+02
3.000000000000000000e+02 -1.003400024414062500e+03
4.000000000000000000e+02 -8.410000000000000000e+02
5.000000000000000000e+02 -8.097600097656250000e+02
6.000000000000000000e+02 -8.418400024414062273e+02
7.000000000000000000e+02 -8.096000000000000227e+02
8.000000000000000000e+02 -8.419599975585937273e+02
9.000000000000000000e+02 -8.415999877929687045e+02
1.000000000000000000e+03 -8.095999877929687045e+02
1.100000000000000000e+03 -8.097199951171875227e+02
1.200000000000000000e+03 -7.775599975585937500e+02
1.300000000000000000e+03 -8.095199951171874773e+02
1.400000000000000000e+03 -7.775599975585937500e+02
1.500000000000000000e+03 -8.420400024414062727e+02
1.600000000000000000e+03 -9.062000000000000455e+02
1.700000000000000000e+03 -9.706000000000000227e+02
1.800000000000000000e+03 -9.383999999999999773e+02
1.900000000000000000e+03 -9.062400024414062045e+02
2.000000000000000000e+03 -8.419199951171874545e+02
2.100000000000000000e+03 -8.420799926757812273e+02
2.200000000000000000e+03 -8.419599853515625227e+02
2.300000000000000000e+03 -8.740399902343749545e+02
2.400000000000000000e+03 -9.063599853515625000e+02
2.500000000000000000e+03 -9.385199829101562727e+02
2.600000000000000000e+03 -9.063999877929687727e+02
2.700000000000000000e+03 -9.062399902343750000e+02
2.800000000000000000e+03 -8.741599853515624545e+02
2.900000000000000000e+03 -9.063599853515625000e+02
3.000000000000000000e+03 -8.739599853515625227e+02
3.100000000000000000e+03 -8.739599853515625227e+02
3.200000000000000000e+03 -8.098799926757812955e+02
3.300000000000000000e+03 -7.456000000000000227e+02
3.400000000000000000e+03 -7.131200073242187045e+02
3.500000000000000000e+03 -7.775200073242187955e+02
3.600000000000000000e+03 -7.453999999999999773e+02
3.700000000000000000e+03 -8.094399902343750455e+02
3.800000000000000000e+03 -8.737199829101562045e+02
3.900000000000000000e+03 -8.737999755859375455e+02
4.000000000000000000e+03 -8.094399780273437273e+02
4.100000000000000000e+03 -7.771999877929687273e+02
4.200000000000000000e+03 -6.809999877929687955e+02
4.300000000000000000e+03 -6.167599975585937955e+02
4.400000000000000000e+03 -5.525599975585937500e+02
4.500000000000000000e+03 -4.883599975585937614e+02
4.600000000000000000e+03 -4.562399902343750000e+02
4.700000000000000000e+03 -4.883599975585937614e+02
4.800000000000000000e+03 -4.883999877929687727e+02
4.900000000000000000e+03 -4.562399902343750000e+02
5.000000000000000000e+03 -4.562399902343750000e+02
}\obstaclenoshieldREINFORCEObs

\pgfplotstableread{
0.000000000000000000e+00 -1.990000000000000000e+02
1.000000000000000000e+02 9.910000000000000000e+02
2.000000000000000000e+02 9.912000122070312500e+02
3.000000000000000000e+02 9.907999877929687500e+02
4.000000000000000000e+02 9.912000122070312500e+02
5.000000000000000000e+02 7.530400024414062727e+02
6.000000000000000000e+02 9.910400024414062727e+02
7.000000000000000000e+02 9.910000000000000000e+02
8.000000000000000000e+02 9.908799926757812955e+02
9.000000000000000000e+02 9.910000000000000000e+02
1.000000000000000000e+03 9.910400024414062727e+02
1.100000000000000000e+03 9.910800048828125455e+02
1.200000000000000000e+03 9.910000122070312045e+02
1.300000000000000000e+03 9.910000122070312045e+02
1.400000000000000000e+03 9.907600097656250000e+02
1.500000000000000000e+03 9.908800048828125000e+02
1.600000000000000000e+03 9.908800048828125000e+02
1.700000000000000000e+03 9.910000000000000000e+02
1.800000000000000000e+03 9.911600097656249773e+02
1.900000000000000000e+03 9.913200073242187500e+02
2.000000000000000000e+03 9.911200073242187045e+02
2.100000000000000000e+03 9.909200073242187727e+02
2.200000000000000000e+03 9.908000122070312727e+02
2.300000000000000000e+03 9.908000122070312727e+02
2.400000000000000000e+03 9.906400146484375000e+02
2.500000000000000000e+03 9.907600097656250000e+02
2.600000000000000000e+03 9.909600097656250455e+02
2.700000000000000000e+03 9.909600097656250455e+02
2.800000000000000000e+03 9.907999999999999545e+02
2.900000000000000000e+03 9.910799926757812273e+02
3.000000000000000000e+03 9.910799926757812273e+02
3.100000000000000000e+03 9.910799926757812273e+02
3.200000000000000000e+03 9.913199829101562273e+02
3.300000000000000000e+03 9.915199829101562727e+02
3.400000000000000000e+03 9.913199829101562273e+02
3.500000000000000000e+03 9.911599853515624545e+02
3.600000000000000000e+03 9.910799804687500227e+02
3.700000000000000000e+03 9.909199829101562500e+02
3.800000000000000000e+03 9.907999877929687500e+02
3.900000000000000000e+03 9.909599975585937273e+02
4.000000000000000000e+03 9.909599975585937273e+02
4.100000000000000000e+03 9.909199951171874545e+02
4.200000000000000000e+03 9.908400024414062273e+02
4.300000000000000000e+03 9.908800048828125000e+02
4.400000000000000000e+03 9.907599975585937955e+02
4.500000000000000000e+03 9.907599975585937955e+02
4.600000000000000000e+03 9.910000000000000000e+02
4.700000000000000000e+03 9.910000000000000000e+02
4.800000000000000000e+03 9.909199951171874545e+02
4.900000000000000000e+03 9.910400024414062727e+02
5.000000000000000000e+03 9.911600097656249773e+02
}\obstacleshieldREINFORCEStack

\pgfplotstableread{
0.000000000000000000e+00 -8.414000244140625000e+02
1.000000000000000000e+02 -8.420000000000000000e+02
2.000000000000000000e+02 -6.812000122070312500e+02
3.000000000000000000e+02 -3.597999877929687500e+02
4.000000000000000000e+02 -3.597999877929687500e+02
5.000000000000000000e+02 -6.168400024414062273e+02
6.000000000000000000e+02 -5.848400024414062273e+02
7.000000000000000000e+02 -5.204800048828125227e+02
8.000000000000000000e+02 -5.847599975585937955e+02
9.000000000000000000e+02 -5.847200012207031250e+02
1.000000000000000000e+03 -6.812000061035156477e+02
1.100000000000000000e+03 -5.847200012207031250e+02
1.200000000000000000e+03 -6.813200012207031477e+02
1.300000000000000000e+03 -5.849200012207031705e+02
1.400000000000000000e+03 -5.849599975585937273e+02
1.500000000000000000e+03 -4.884799926757812614e+02
1.600000000000000000e+03 -4.884799926757812614e+02
1.700000000000000000e+03 -4.561999877929687273e+02
1.800000000000000000e+03 -3.918799926757812386e+02
1.900000000000000000e+03 -3.918799926757812386e+02
2.000000000000000000e+03 -4.240000000000000000e+02
2.100000000000000000e+03 -4.882800048828124773e+02
2.200000000000000000e+03 -4.240400024414062727e+02
2.300000000000000000e+03 -4.883599975585937614e+02
2.400000000000000000e+03 -4.883200012207031477e+02
2.500000000000000000e+03 -4.883599914550781023e+02
2.600000000000000000e+03 -4.562399841308593977e+02
2.700000000000000000e+03 -4.240799865722656250e+02
2.800000000000000000e+03 -3.919199890136718523e+02
2.900000000000000000e+03 -4.240799926757812273e+02
3.000000000000000000e+03 -4.240799926757812273e+02
3.100000000000000000e+03 -4.240799926757812273e+02
3.200000000000000000e+03 -4.240799926757812273e+02
3.300000000000000000e+03 -4.240799926757812273e+02
3.400000000000000000e+03 -3.919599853515625227e+02
3.500000000000000000e+03 -3.597999877929687500e+02
3.600000000000000000e+03 -3.597999877929687500e+02
3.700000000000000000e+03 -3.276399902343749773e+02
3.800000000000000000e+03 -2.954799926757812614e+02
3.900000000000000000e+03 -2.954799926757812614e+02
4.000000000000000000e+03 -2.954399963378906477e+02
4.100000000000000000e+03 -2.954399963378906477e+02
4.200000000000000000e+03 -3.597599914550781364e+02
4.300000000000000000e+03 -3.597599914550781364e+02
4.400000000000000000e+03 -3.597599914550781364e+02
4.500000000000000000e+03 -3.276399902343749773e+02
4.600000000000000000e+03 -2.954799926757812614e+02
4.700000000000000000e+03 -3.597599975585937386e+02
4.800000000000000000e+03 -3.597599975585937386e+02
4.900000000000000000e+03 -3.597599975585937386e+02
5.000000000000000000e+03 -4.240400024414062727e+02
}\obstaclenoshieldREINFORCEStack

==> figs/data/ShieldSwitching/Normalized/DecayedSwitch.tex <==
\pgfplotstableread{
0.000000000000000000e+00 4.634872251086765149e-01 4.069911207506392015e-01 4.975673576710595292e-01 4.135106012556288291e-01 5.075711741977267932e-01 3.124182209391054288e-01 6.145562292782474900e-01
1.000000000000000000e+02 8.311795898013644157e-01 8.602298223626031470e-01 8.742212723626030524e-01 7.416062560611301757e-01 8.754565775129531380e-01 6.801105856317933851e-01 9.822485939709354463e-01
2.000000000000000000e+02 8.223545877668593240e-01 7.876379390292697069e-01 8.734841390292698016e-01 7.302951471540662931e-01 8.753649739159478083e-01 6.712855835972882934e-01 9.734235919364303546e-01
3.000000000000000000e+02 8.218462513817681447e-01 7.877092473626031710e-01 9.718784390292696473e-01 7.799952127668592361e-01 8.636972899966769424e-01 6.707772472121971141e-01 9.729152555513391754e-01
4.000000000000000000e+02 8.563129211001926366e-01 8.728493390292696441e-01 9.741379390292697282e-01 8.218053069644503106e-01 8.754021595848930914e-01 7.052439169306214950e-01 1.007381925269763778e+00
5.000000000000000000e+02 9.090361150317721517e-01 7.930834937068769852e-01 9.482578294242944628e-01 6.974425048404270244e-01 7.994984350416395325e-01 4.168302763832940627e-01 6.413888888888888973e-01
6.000000000000000000e+02 9.316862034691703265e-01 8.165961304237194796e-01 9.709698214555442464e-01 7.714982834710015780e-01 8.707731606377495659e-01 5.805560022897110484e-01 6.413888888888888973e-01
7.000000000000000000e+02 9.361278214348687454e-01 8.167917925914087718e-01 9.687008665726047019e-01 7.884936238182915780e-01 8.686314724816216470e-01 5.833141628905593734e-01 6.413888888888888973e-01
8.000000000000000000e+02 9.388461042616102148e-01 8.288814216766442478e-01 9.664817410675134113e-01 8.015717027876112510e-01 8.664237319522433145e-01 6.043267303777885013e-01 6.394554826213435517e-01
9.000000000000000000e+02 9.331693872663711309e-01 8.265098900783369729e-01 9.474552346279992099e-01 7.972102644178603592e-01 8.594317360772026904e-01 6.045392699098625089e-01 6.338161738326776318e-01
1.000000000000000000e+03 9.273810047997368633e-01 9.070912690227848296e-01 9.450483045248752267e-01 7.897772685580782825e-01 8.572347438388400187e-01 6.154633990050252246e-01 6.182119452502102819e-01
1.100000000000000000e+03 9.292010039859348813e-01 8.216622256690554460e-01 9.453124013426291938e-01 7.921381914350721365e-01 8.573403701358369711e-01 6.161703633681675507e-01 6.177849796663649196e-01
1.200000000000000000e+03 9.240126692030166344e-01 8.045240813525985635e-01 9.451460715628136278e-01 7.836484829796684926e-01 8.574114793989392469e-01 6.161331200103064010e-01 6.178622201250559831e-01
1.300000000000000000e+03 9.225660015953911719e-01 8.073244418646580156e-01 9.453055261711458490e-01 7.731598435295952143e-01 8.575292343987358512e-01 5.929841203168666475e-01 6.178578829756410373e-01
1.400000000000000000e+03 8.766767103407101750e-01 8.215477944657475495e-01 9.624792384112632826e-01 7.672479808383517730e-01 8.646228399488661287e-01 5.856186486167404004e-01 6.180217960235702135e-01
1.500000000000000000e+03 8.293176687452527007e-01 8.358209757918378946e-01 8.626075933011710939e-01 7.693116651746962908e-01 8.646090935601128402e-01 5.852287269463501973e-01 6.182117131163236134e-01
1.600000000000000000e+03 8.258876706017387326e-01 8.214070695168388392e-01 8.625362855105929150e-01 7.651316572401259952e-01 8.642507620069715957e-01 5.851212515973838180e-01 6.181858584380276467e-01
1.700000000000000000e+03 8.207443385654026313e-01 8.213120453488752526e-01 8.623622335443453801e-01 7.499549239688448887e-01 8.636049471113417253e-01 5.817984375810404396e-01 6.179286744380136920e-01
1.800000000000000000e+03 8.204226723564995716e-01 8.040005232802412971e-01 8.620313021592541647e-01 7.582003837161593873e-01 8.634750482771131885e-01 5.855074966177439277e-01 6.173862846111083380e-01
1.900000000000000000e+03 8.091976686689589249e-01 7.888199561118147685e-01 8.439098262555271290e-01 7.596929847293431015e-01 8.453682492150201844e-01 5.923491151686844924e-01 6.176795565198192062e-01
2.000000000000000000e+03 8.007993339114719555e-01 7.743656740841758923e-01 8.437598256026798138e-01 7.374448991987440083e-01 8.453674699995251673e-01 5.656981060349676182e-01 6.176705619914267809e-01
2.100000000000000000e+03 8.060043357425265009e-01 7.914701486131118235e-01 8.438478000599246576e-01 7.443304862552219126e-01 8.457646572960747511e-01 5.657256749368338999e-01 6.177296630114353926e-01
2.200000000000000000e+03 8.128159977806937997e-01 8.060670506817458891e-01 8.441070832831657489e-01 7.618317748599583439e-01 8.461334167056612232e-01 5.690465040652535889e-01 6.177354914961342702e-01
2.300000000000000000e+03 8.163159977806939693e-01 8.230763365163760170e-01 8.442333720184665991e-01 7.668241577996148806e-01 8.461981357150607508e-01 5.689812472697494128e-01 6.178940812180706565e-01
2.400000000000000000e+03 8.308826653374565829e-01 8.384374931727430758e-01 8.621814697373538783e-01 7.785878715091282265e-01 8.643725483788383679e-01 5.697361448174463883e-01 6.177725187838990495e-01
2.500000000000000000e+03 8.359060008578831358e-01 8.530227074585045033e-01 8.620555166855959905e-01 7.875511106703015907e-01 8.642581353081597584e-01 5.930000951217592187e-01 6.178085740744756471e-01
2.600000000000000000e+03 8.307943327162000680e-01 8.360015677887809860e-01 8.621649705309888390e-01 7.807794314914279221e-01 8.639337080213757014e-01 5.928640610810819167e-01 6.180646057754718425e-01
2.700000000000000000e+03 8.290726653628879284e-01 8.213665215137820885e-01 8.620866136825391379e-01 7.784038313123914365e-01 8.639806117587619516e-01 5.927298390601639655e-01 6.181188272369008141e-01
2.800000000000000000e+03 8.272209982130264150e-01 8.184950176273938505e-01 8.619438250880261387e-01 7.755442247602674088e-01 8.638528055402967532e-01 5.927163535557856688e-01 6.178656463289257106e-01
2.900000000000000000e+03 8.323493317498101840e-01 8.211147865828789527e-01 8.619909134443495269e-01 7.886385996076796800e-01 8.633960934533012610e-01 5.926042061219098933e-01 6.178844608363691648e-01
3.000000000000000000e+03 8.305593298170300676e-01 8.065536227374860978e-01 8.617910839564090208e-01 7.962949220869276479e-01 8.611967630598279522e-01 6.151482840726013590e-01 6.178937123534511411e-01
3.100000000000000000e+03 8.307293287489149192e-01 8.236058595142449201e-01 8.617768215268029053e-01 7.865526121351454902e-01 8.615141615125868624e-01 5.694734563092183066e-01 6.176685385909553849e-01
3.200000000000000000e+03 8.274059962802463586e-01 8.236534560401239657e-01 8.617768222897423946e-01 7.732807378980849355e-01 8.615510737948947062e-01 5.662216710533658492e-01 6.177003251692362307e-01
3.300000000000000000e+03 8.140293320549858436e-01 8.095155054282718865e-01 8.473012343276807856e-01 7.464559341006808957e-01 8.572775530073378780e-01 5.540830382264528842e-01 6.177976012944607076e-01
3.400000000000000000e+03 8.053993304782443019e-01 7.923108628885735527e-01 8.471919511044395668e-01 7.292844717237684238e-01 8.571890127393934078e-01 5.540262789607998117e-01 6.178343588307843026e-01
3.500000000000000000e+03 8.088893319023980899e-01 7.924416254999627762e-01 8.475916152007122450e-01 7.328085119459365471e-01 8.594538666619194744e-01 5.540861753355029728e-01 6.178611323779560349e-01
3.600000000000000000e+03 8.153309969160292825e-01 7.922821706714460177e-01 8.473343939871044173e-01 7.525970551384819629e-01 8.591803602430555520e-01 5.650190297758976854e-01 6.178962996274497410e-01
3.700000000000000000e+03 8.203443292829725175e-01 8.066723628501722976e-01 8.472725389564090825e-01 7.681566215091281125e-01 8.593239926232231207e-01 5.682722617864496284e-01 6.180963986105502128e-01
3.800000000000000000e+03 8.338426609887017449e-01 8.212383340841759027e-01 8.618812926814100051e-01 7.950153810713027625e-01 8.636593802981905599e-01 6.158040774399649031e-01 6.179779130351599203e-01
3.900000000000000000e+03 8.389976621839734250e-01 8.381383326683891077e-01 8.618336971386547640e-01 8.017909348381889734e-01 8.641463216993542362e-01 6.159089430498091433e-01 6.179530479848046598e-01
4.000000000000000000e+03 8.423476618025037554e-01 8.550333537923008320e-01 8.618216706127759252e-01 8.066928178999158705e-01 8.640474748823376849e-01 6.158912467622291720e-01 6.178440772496794908e-01
4.100000000000000000e+03 8.356409944746229224e-01 8.523402104589674622e-01 8.618027713143242563e-01 7.872867582533095154e-01 8.642403127882215541e-01 5.930930312919501235e-01 6.175622934320352808e-01
4.200000000000000000e+03 8.288543314192029499e-01 8.379214941839684405e-01 8.615577469184705350e-01 7.698144938998753295e-01 8.636896523369683720e-01 5.855065186474345262e-01 6.171472481872933846e-01
4.300000000000000000e+03 8.270376647525363722e-01 8.232414277681817660e-01 8.613888423895348367e-01 7.675636443667942510e-01 8.635978723737928187e-01 5.854979442083076968e-01 6.170624896999880038e-01
4.400000000000000000e+03 8.288193311903211402e-01 8.234484765034825182e-01 8.616123901110160910e-01 7.711167771233452539e-01 8.635355230543347860e-01 5.855196366888831827e-01 6.170741313156852259e-01
4.500000000000000000e+03 8.254876638624403240e-01 8.234701215034824218e-01 8.614173680116864462e-01 7.577635549757215649e-01 8.636392751905653808e-01 5.821967316515435087e-01 6.171370342167944445e-01
4.600000000000000000e+03 8.289793343438042195e-01 8.236556923765142590e-01 8.616127292866856413e-01 7.711809310489230462e-01 8.637734997643363721e-01 5.852468487685477117e-01 6.175735885475440723e-01
4.700000000000000000e+03 8.357843337588840571e-01 8.381788798061200474e-01 8.619886811428408846e-01 7.886456996493867999e-01 8.642037646823458319e-01 5.930893473759121237e-01 6.175726530682882354e-01
4.800000000000000000e+03 8.375293340894911509e-01 8.526281831701489899e-01 8.621077534623547978e-01 7.908242955101861815e-01 8.643013287438287007e-01 5.931169141759747854e-01 6.175584186351688043e-01
4.900000000000000000e+03 8.323359977298312451e-01 8.355591115034823879e-01 8.620101555206892696e-01 7.823673895094129804e-01 8.642225111219618006e-01 5.928900140496270454e-01 6.176719777479261486e-01
5.000000000000000000e+03 8.322976656172010879e-01 8.185378009914229258e-01 8.621053438847181560e-01 7.906884107801649408e-01 8.642238872104219816e-01 6.161469119772166048e-01 6.176484172226803793e-01
}\SwitchShieldNormSoft


==> figs/data/ShieldSwitching/Normalized/HardSwitch.tex <==
\pgfplotstableread{
0.000000000000000000e+00 6.083142649332682339e-01 6.036160860125223682e-01 6.123456005700429472e-01 5.989672931035360248e-01 6.176612288157145025e-01 4.162666884762042385e-01 8.003618413903321738e-01
1.000000000000000000e+02 8.636305335362752800e-01 8.445917052347819975e-01 9.317858103939055114e-01 7.852944606145223494e-01 9.268772586186727613e-01 6.715829570792112291e-01 1.055678109993339220e+00
2.000000000000000000e+02 8.546721801757812820e-01 8.313270267270406189e-01 9.314782196746825838e-01 7.712911148071288636e-01 9.263662974039714726e-01 6.626246037187172311e-01 1.046719756632845000e+00
3.000000000000000000e+02 8.462221806844075767e-01 8.318751425362904683e-01 9.315229349969227357e-01 7.128687677383424015e-01 9.348589595158894872e-01 6.541746042273436368e-01 1.038269757141471628e+00
4.000000000000000000e+02 9.057888580958048497e-01 7.734120548377991122e-01 9.752136723884581970e-01 5.222031927108764515e-01 6.774895264307657650e-01 4.137412816387408543e-01 7.978364345528689006e-01
5.000000000000000000e+02 8.557256034851073112e-01 8.369644030696869130e-01 9.164692476048025505e-01 6.781249657948813514e-01 8.166506541570028865e-01 4.513838805647167884e-01 7.524999999999999467e-01
6.000000000000000000e+02 8.549938497543334792e-01 8.311373505597432709e-01 9.285141622320555399e-01 6.627085157394408954e-01 8.282170530319213908e-01 5.195926273128398387e-01 6.898750730096291361e-01
7.000000000000000000e+02 9.036005146662395182e-01 8.626351123671977428e-01 9.775138293800862854e-01 6.097254141489664159e-01 7.789462832132975079e-01 5.194894903374395190e-01 6.900648735490756414e-01
8.000000000000000000e+02 8.736071813583374146e-01 8.319304940031686968e-01 9.440634914000193723e-01 5.807767962773641157e-01 7.472048877080280649e-01 5.194588831926028050e-01 6.900154801344234867e-01
9.000000000000000000e+02 8.504021801630656130e-01 8.151663969652302333e-01 9.109493944798787046e-01 5.709451791127522213e-01 7.141584070841471288e-01 5.192489162428740590e-01 5.233454434729055693e-01
1.000000000000000000e+03 8.632971744537353720e-01 8.359947713430785798e-01 9.117751686195372685e-01 5.843920982996623215e-01 7.257553864161173651e-01 5.180522035017108839e-01 5.232688102668029417e-01
1.100000000000000000e+03 6.849671753565470533e-01 6.566813746457164092e-01 9.302107399252318887e-01 6.087388294219969742e-01 7.440455926259358366e-01 5.182336617619337504e-01 5.231940204788702031e-01
1.200000000000000000e+03 7.009721710840860487e-01 6.747098948171995625e-01 7.475753310618337144e-01 6.248908500671386257e-01 7.613177846272786153e-01 5.195956450494928491e-01 5.221253619797227019e-01
1.300000000000000000e+03 6.973105016708375237e-01 6.719267058617147681e-01 7.471938907519531936e-01 6.205860198974609832e-01 7.589964347839356362e-01 5.196358442796266131e-01 5.216784905897581259e-01
1.400000000000000000e+03 6.973671680450439503e-01 6.724765388340757655e-01 7.470078191185760552e-01 6.207312696456909196e-01 7.589003510157268373e-01 5.196621606155730211e-01 5.216321757033967055e-01
1.500000000000000000e+03 7.075721681594848711e-01 6.726244705007425884e-01 7.639320366966755316e-01 6.333928727467854625e-01 7.655850776672363800e-01 5.205518094778156524e-01 5.216225266377034764e-01
1.600000000000000000e+03 7.093388378143310469e-01 6.725215587546792273e-01 7.642892609620411948e-01 6.351448001225790119e-01 7.662999287287394212e-01 5.202412424522228074e-01 5.221464337867908201e-01
1.700000000000000000e+03 7.162538370132446319e-01 7.038588401704660713e-01 7.644841118964640359e-01 6.442907036463420001e-01 7.666382019678752435e-01 5.201814714664234618e-01 5.221462027635163095e-01
1.800000000000000000e+03 7.198755051930745275e-01 7.040538659744007832e-01 7.650224265047963490e-01 6.477868448257446676e-01 7.691585538864135208e-01 5.204501661313908345e-01 5.220308430340551142e-01
1.900000000000000000e+03 7.169338434855142550e-01 6.898038924311827857e-01 7.654841215944925281e-01 6.410520331064860633e-01 7.697566603342691494e-01 5.193682188326266269e-01 5.237794659004463282e-01
2.000000000000000000e+03 7.168788431167602004e-01 7.038105815274556809e-01 7.655059349278259262e-01 6.398398128509521499e-01 7.697376818339028981e-01 5.193576437836940896e-01 5.237833747659071948e-01
2.100000000000000000e+03 7.100221748987833870e-01 7.013009408439127013e-01 7.651298088550059218e-01 6.276154407501221000e-01 7.694307802836100052e-01 5.192064475109822164e-01 5.237012323647095569e-01
2.200000000000000000e+03 7.031188408533731726e-01 6.699136586651865954e-01 7.649466441852824650e-01 6.184760259628295787e-01 7.690631907780964838e-01 5.191365635577308568e-01 5.237244498547447558e-01
2.300000000000000000e+03 7.031905108769734847e-01 6.726568029816437644e-01 7.648514566942851145e-01 6.193422591527303345e-01 7.687834891637166379e-01 5.192740638498732908e-01 5.238069558695684913e-01
2.400000000000000000e+03 7.008538377126058982e-01 6.697256792053476460e-01 7.640565932302602059e-01 6.176007315317789681e-01 7.681429724375407053e-01 5.203415867242684456e-01 5.220060860560863381e-01
2.500000000000000000e+03 6.987771652221680396e-01 6.552763698478952792e-01 7.634631287857054360e-01 6.152557730992634921e-01 7.676742389043171855e-01 5.188787161610992626e-01 5.229222787119475191e-01
2.600000000000000000e+03 7.002871569951375497e-01 6.552380543665313750e-01 7.631749762970988504e-01 6.168460279464721419e-01 7.671731087366739921e-01 5.181668402910966087e-01 5.230408070325117675e-01
2.700000000000000000e+03 7.018521507898966005e-01 6.721758588544718416e-01 7.629083030865477788e-01 6.161519264221191339e-01 7.667289666493734002e-01 5.177415667360633078e-01 5.229794015103966798e-01
2.800000000000000000e+03 6.945888062795003703e-01 6.547595207924143956e-01 7.620615387417856157e-01 6.075460336685180041e-01 7.639353996912637834e-01 5.182137711842854655e-01 5.216938432057698360e-01
2.900000000000000000e+03 6.979071336110432844e-01 6.717493920878091496e-01 7.623136004211424899e-01 6.124830796559651569e-01 7.634492056528726645e-01 5.196638011932372958e-01 5.196638011932372958e-01
3.000000000000000000e+03 6.963004675547281863e-01 6.719255104211425689e-01 7.625349087544758264e-01 6.125479381561279579e-01 7.610621501922607557e-01 5.196638011932372958e-01 5.196638011932372958e-01
3.100000000000000000e+03 6.996521338144937596e-01 6.744215637544760389e-01 7.625656687544758450e-01 6.197819911956786720e-01 7.610625733693442418e-01 5.196638011932372958e-01 5.196638011932372958e-01
3.200000000000000000e+03 6.927038010915119726e-01 6.573885670878092391e-01 7.478354354211425026e-01 6.158487168629964703e-01 7.564844209035238576e-01 5.188304678599039432e-01 5.196638011932372958e-01
3.300000000000000000e+03 6.961338003794351748e-01 6.743765420878092831e-01 7.480651854211425311e-01 6.185884009043375320e-01 7.575222433725992133e-01 5.188304678599039432e-01 5.196638011932372958e-01
3.400000000000000000e+03 6.840354666392008953e-01 6.427064337544758921e-01 7.474442137544757836e-01 6.044550156911214778e-01 7.530824331919352410e-01 5.196638011932372958e-01 5.196638011932372958e-01
3.500000000000000000e+03 6.840471330006917539e-01 6.424755054211425120e-01 7.475777154211424858e-01 6.025237082163493740e-01 7.551179719289144998e-01 5.188304678599039432e-01 5.196638011932372958e-01
3.600000000000000000e+03 6.804971340179443162e-01 6.421920037544758264e-01 7.472069120878092052e-01 5.990255819956461503e-01 7.529032492319743808e-01 5.188304678599039432e-01 5.196638011932372958e-01
3.700000000000000000e+03 6.907371344248454115e-01 6.593868570878091973e-01 7.617727154211425544e-01 6.104614742279053097e-01 7.578786093393961032e-01 5.179971345265705907e-01 5.196638011932372958e-01
3.800000000000000000e+03 6.975538016001383568e-01 6.594772370878092538e-01 7.619706470878092608e-01 6.261731497446696437e-01 7.588827607472737879e-01 5.188304678599039432e-01 5.196638011932372958e-01
3.900000000000000000e+03 7.077871349334716733e-01 6.764933987544758942e-01 7.622490020878092132e-01 6.379859706878662218e-01 7.633176179250081850e-01 5.188304678599039432e-01 5.196638011932372958e-01
4.000000000000000000e+03 7.112404689788819345e-01 6.909664170878092593e-01 7.624440237544759524e-01 6.421366374969482704e-01 7.636729056040446606e-01 5.196638011932372958e-01 5.196638011932372958e-01
4.100000000000000000e+03 7.095388019561768012e-01 6.911141804211425876e-01 7.481629487544759760e-01 6.410440514882406182e-01 7.612463156382243135e-01 5.188304678599039432e-01 5.196638011932372958e-01
4.200000000000000000e+03 7.096388009389240636e-01 7.026423237544759948e-01 7.485701637544758258e-01 6.405831933339436457e-01 7.612497366587320791e-01 5.188304678599039432e-01 5.196638011932372958e-01
4.300000000000000000e+03 7.114754673004149987e-01 7.171131054211424827e-01 7.489555654211424995e-01 6.381066771189370934e-01 7.618441214243570903e-01 5.196638011932372958e-01 5.196638011932372958e-01
4.400000000000000000e+03 7.096721337636311411e-01 7.144584420878091757e-01 7.486937087544759395e-01 6.353719532012940263e-01 7.618403504689533756e-01 5.196638011932372958e-01 5.196638011932372958e-01
4.500000000000000000e+03 7.080554660797120370e-01 7.002069004211426417e-01 7.487151854211425706e-01 6.331590503692626770e-01 7.618318289438882340e-01 5.196638011932372958e-01 5.196638011932372958e-01
4.600000000000000000e+03 7.028921326955158699e-01 6.832450437544759225e-01 7.626819987544758428e-01 6.259193187713623097e-01 7.618474102020265093e-01 5.196638011932372958e-01 5.196638011932372958e-01
4.700000000000000000e+03 7.064038005828857658e-01 6.862048537544759297e-01 7.627699737544758607e-01 6.321110688527423749e-01 7.618341431935627961e-01 5.196638011932372958e-01 5.196638011932372958e-01
4.800000000000000000e+03 7.028704672495523775e-01 6.836924704211425619e-01 7.625342354211426255e-01 6.259421047210692590e-01 7.618341431935627961e-01 5.196638011932372958e-01 5.196638011932372958e-01
4.900000000000000000e+03 7.029471345265706494e-01 6.837637787544759149e-01 7.626058804211425235e-01 6.259703787485758619e-01 7.618379141489665107e-01 5.196638011932372958e-01 5.196638011932372958e-01
5.000000000000000000e+03 6.960904679616293222e-01 6.666804454211425757e-01 7.623371454211426146e-01 6.172057257334391256e-01 7.612743083953857903e-01 5.196638011932372958e-01 5.196638011932372958e-01
}\SwitchShieldNormHard


==> figs/data/ShieldSwitching/Normalized/NoShield.tex <==
\pgfplotstableread{
0.000000000000000000e+00 4.202962572309705269e-01 4.319032223626030897e-01 4.434712723626030861e-01 3.483843271467421121e-01 4.922081911298963330e-01 3.694089147178420962e-01 4.711835997440991242e-01
1.000000000000000000e+02 3.622135183546278392e-01 3.033257228948805229e-01 4.158364890273623105e-01 2.480031568739149428e-01 4.620162133110894409e-01 3.113261758414992975e-01 4.131008608677563809e-01
2.000000000000000000e+02 3.831469760470919694e-01 3.075783987928602525e-01 4.865795527002546028e-01 2.357486046685113024e-01 4.939458779229057850e-01 3.322596335339635387e-01 4.340343185602205112e-01
3.000000000000000000e+02 4.125384072197808005e-01 4.439054828002506059e-01 4.786875967966291445e-01 2.789339569939507379e-01 5.215986794365776724e-01 3.616510647066523698e-01 4.634257497329093423e-01
4.000000000000000000e+02 4.047801941765680200e-01 3.956110596073998398e-01 4.177034131829155394e-01 2.985425321790907138e-01 4.955470564100477593e-01 3.538928516634394783e-01 4.556675366896964507e-01
5.000000000000000000e+02 3.965950706058078978e-01 3.764647772915987733e-01 4.484556648139529922e-01 2.819225155724419118e-01 4.930632036421033759e-01 4.480910502155544539e-01 4.747222222222222121e-01
6.000000000000000000e+02 3.932851530287000963e-01 3.678300265731896945e-01 4.545267091706170492e-01 2.696110269758436595e-01 4.955809922112358046e-01 4.704145513860811811e-01 4.738888888888888595e-01
7.000000000000000000e+02 3.992534759097629560e-01 3.810770828888532802e-01 4.677208263442314551e-01 2.702948175642225226e-01 5.045272553337944998e-01 4.700748555173462351e-01 4.730555555555555625e-01
8.000000000000000000e+02 4.009933608068360633e-01 3.900521843943108302e-01 4.634735907465701854e-01 2.818520991696251698e-01 5.028710483544402976e-01 4.574210725678330980e-01 4.730555555555555625e-01
9.000000000000000000e+02 3.994966853790813399e-01 3.769872339020368668e-01 4.489955851784345753e-01 2.899634278032514612e-01 4.947543979638152067e-01 4.569966442746430935e-01 4.738888888888888595e-01
1.000000000000000000e+03 4.023116498006715225e-01 3.750069332511732356e-01 4.602672924488406259e-01 2.892877528561486056e-01 4.995668674462371839e-01 4.590311414155126002e-01 4.738888888888888595e-01
1.100000000000000000e+03 4.066949897461467067e-01 3.877081398640273568e-01 4.598585527122836525e-01 2.982852792792849983e-01 4.995305487308237535e-01 4.590252035867160019e-01 4.747222222222222121e-01
1.200000000000000000e+03 4.084449603729777833e-01 3.861511059945254565e-01 4.591088726019880162e-01 3.003168614122602720e-01 5.014397818240854399e-01 4.605410908076211229e-01 4.747222222222222121e-01
1.300000000000000000e+03 4.217617161009046267e-01 4.068369214545779489e-01 4.787086505827415905e-01 3.064284813774956762e-01 5.178870784335666277e-01 4.705769866939898960e-01 4.747222222222222121e-01
1.400000000000000000e+03 4.143767374250623692e-01 3.911713606387668407e-01 4.937041763840823161e-01 2.916125335269504348e-01 5.160843232048882845e-01 4.708372389365365618e-01 4.747222222222222121e-01
1.500000000000000000e+03 4.058633985731336380e-01 3.711872984058210423e-01 4.934185514584180088e-01 2.814814086490207146e-01 5.095705246819389744e-01 4.698624615869778087e-01 4.747222222222222121e-01
1.600000000000000000e+03 4.063334019554985521e-01 3.710678367519718024e-01 4.948200988629743446e-01 2.727658992343478528e-01 5.170886635674371012e-01 4.701622016358340539e-01 4.738888888888888595e-01
1.700000000000000000e+03 4.140984609815809847e-01 3.779367835991500058e-01 4.985940331465486541e-01 2.809442037794324665e-01 5.225378467135959326e-01 4.699063072860615864e-01 4.738888888888888595e-01
1.800000000000000000e+03 4.025217467202080734e-01 3.601948467387983688e-01 4.826352718334791514e-01 2.713918718549940823e-01 5.100597858005099239e-01 4.654106926584097859e-01 4.733072635586100252e-01
1.900000000000000000e+03 4.167934478335910686e-01 3.799900346425205133e-01 4.825240855738914814e-01 2.835189858330620649e-01 5.230990586174858459e-01 4.629895567369805565e-01 4.730555555555555625e-01
2.000000000000000000e+03 4.219834128909640825e-01 3.968088010959201495e-01 4.826042224630821553e-01 2.884840008629692698e-01 5.296079254998100616e-01 4.563986901990666478e-01 4.730555555555555625e-01
2.100000000000000000e+03 4.189017441643609341e-01 3.782986301175774169e-01 4.850508292013125389e-01 2.821970696343316098e-01 5.302481708102756430e-01 4.561245837057494867e-01 4.730555555555555625e-01
2.200000000000000000e+03 4.094983413034015141e-01 3.751621467191907366e-01 4.668904700735303503e-01 2.861267676128281257e-01 5.130853050086233713e-01 4.561545566938229324e-01 4.738888888888888595e-01
2.300000000000000000e+03 4.076733371708127773e-01 3.751929407471041866e-01 4.651622438518099867e-01 2.814228663219345283e-01 5.154737345231903412e-01 4.556304989762964275e-01 4.738888888888888595e-01
2.400000000000000000e+03 3.977266697539223461e-01 3.693481706243218476e-01 4.661342964812808520e-01 2.709135381155543532e-01 5.073287788245411933e-01 4.549785397477921767e-01 4.738888888888888595e-01
2.500000000000000000e+03 3.902650553994708726e-01 3.544272598139530661e-01 4.667985732966443702e-01 2.655641610556178089e-01 4.978075792802704735e-01 4.607432894315540151e-01 4.738888888888888595e-01
2.600000000000000000e+03 4.024534133248858780e-01 3.764393794921196967e-01 4.797845929736666570e-01 2.844779951824081832e-01 5.029906799170705822e-01 4.610067780421463479e-01 4.747222222222222121e-01
2.700000000000000000e+03 4.109984700732761120e-01 3.805261498054843816e-01 4.956449331639691813e-01 2.836761579725477489e-01 5.156389771355521789e-01 4.655912128789364002e-01 4.747222222222222121e-01
2.800000000000000000e+03 4.099518242094251641e-01 3.677865479753197331e-01 4.958129987323082744e-01 2.868734475029839359e-01 5.088047399732801290e-01 4.700273024143686862e-01 4.747222222222222121e-01
2.900000000000000000e+03 4.095633953306410113e-01 3.633570986518690482e-01 4.916049657536145645e-01 2.839113573286268788e-01 5.144042160881890924e-01 4.627386369876695382e-01 4.738888888888888595e-01
3.000000000000000000e+03 4.144600647184584208e-01 3.798113639695824273e-01 4.923492827892896884e-01 2.881324326409234193e-01 5.178964000278049040e-01 4.628471197512459834e-01 4.738888888888888595e-01
3.100000000000000000e+03 4.030616837395561980e-01 3.613797329672580605e-01 4.776014862916395098e-01 2.717553343031141599e-01 5.124905831231011399e-01 4.612532474888609291e-01 4.738888888888888595e-01
3.200000000000000000e+03 4.030549862119887083e-01 3.731639538190036354e-01 4.770756926458316616e-01 2.758791731092664623e-01 5.098478257073296716e-01 4.643600179836322450e-01 4.738888888888888595e-01
3.300000000000000000e+03 4.037000029457940009e-01 3.840744517302279726e-01 4.775896297350650244e-01 2.751739538404676666e-01 5.115768794589572455e-01 4.634730408245353872e-01 4.738888888888888595e-01
3.400000000000000000e+03 4.130083664152357503e-01 3.895850221476830910e-01 4.829076106396059664e-01 2.862336566501193502e-01 5.168597039116753500e-01 4.695705594326364252e-01 4.738888888888888595e-01
3.500000000000000000e+03 4.194466675016614854e-01 4.017501061967807541e-01 4.821164909211053118e-01 2.927755146874321812e-01 5.239488322787814178e-01 4.673299617818626461e-01 4.747222222222222121e-01
3.600000000000000000e+03 4.198800537957085299e-01 4.015242716587406058e-01 4.821502441168551978e-01 2.974592760297987137e-01 5.186179858737521853e-01 4.670182193849322094e-01 4.738888888888888595e-01
3.700000000000000000e+03 4.230667572869195037e-01 3.886980725099266620e-01 4.845856674347771009e-01 2.940352289411756748e-01 5.271585615370009137e-01 4.654760765997814631e-01 4.738888888888888595e-01
3.800000000000000000e+03 4.270400739881727303e-01 3.890309288661786824e-01 4.837995257270388816e-01 2.969857268863254074e-01 5.320208395216200481e-01 4.645932968760378423e-01 4.747222222222222121e-01
3.900000000000000000e+03 4.297067757500542817e-01 4.067909099222903890e-01 4.826991980213757860e-01 3.054352974785699004e-01 5.272024829440646876e-01 4.668547348532123276e-01 4.747222222222222121e-01
4.000000000000000000e+03 4.210601223839653962e-01 3.926455252223290393e-01 4.699318102331373481e-01 3.015910267723930782e-01 5.164708873324924676e-01 4.702185301713364129e-01 4.747222222222222121e-01
4.100000000000000000e+03 4.175901240878635012e-01 3.917671989096662699e-01 4.700620682694837682e-01 2.946404461754693060e-01 5.155949603610568976e-01 4.701818009323718850e-01 4.738888888888888595e-01
4.200000000000000000e+03 4.023684309217665511e-01 3.580262112336816127e-01 4.667211408933596428e-01 2.768553245120578543e-01 5.046967967563206203e-01 4.712873919118523713e-01 4.738888888888888595e-01
4.300000000000000000e+03 4.072350937737359011e-01 3.759964914518059698e-01 4.667002170811292427e-01 2.822177503797743126e-01 5.098891688876682204e-01 4.704232398300752238e-01 4.738888888888888595e-01
4.400000000000000000e+03 3.867966969384087350e-01 3.384271075070275359e-01 4.489143714759657455e-01 2.611495217217339460e-01 4.956685120476616579e-01 4.623553974677077072e-01 4.741367977386531929e-01
4.500000000000000000e+03 4.034534134758842594e-01 3.549004960206943449e-01 4.795115773492007460e-01 2.720782587263319008e-01 5.136605235629611022e-01 4.618254698513380441e-01 4.738888888888888595e-01
4.600000000000000000e+03 4.080600832197400774e-01 3.722362712250603667e-01 4.791473072902001085e-01 2.839024426354302411e-01 5.118828476799858196e-01 4.618254653015038680e-01 4.747222222222222121e-01
4.700000000000000000e+03 4.172367819044324744e-01 3.895282584631941103e-01 4.799174065275912393e-01 2.929791912926567599e-01 5.184951404147678522e-01 4.602434511327812561e-01 4.747222222222222121e-01
4.800000000000000000e+03 4.110751609378390792e-01 3.617874809110853129e-01 4.817827209419843215e-01 2.887523949517143973e-01 5.081433408949110886e-01 4.628460757911430079e-01 4.747222222222222121e-01
4.900000000000000000e+03 4.233718794080945647e-01 3.821666256697930364e-01 4.974685184819624406e-01 2.989706496768527733e-01 5.189348867628309492e-01 4.722222222222221544e-01 4.747222222222222121e-01
5.000000000000000000e+03 4.079601925743950308e-01 3.650295443761275016e-01 4.804618075142499944e-01 2.834377297295464504e-01 5.063537710401747605e-01 4.722222222222221544e-01 4.738888888888888595e-01
}\SwitchShieldNormNoShield


==> figs/data/ShieldSwitching/Normalized/Shield.tex <==
\pgfplotstableread{
0.000000000000000000e+00	6.486205802493630000e-01	5.727797006532880000e-01	6.614945256413350000e-01	5.358105216556120000e-01	7.098888888888890000e-01	5.540684401862840000e-01	7.431727203124420000e-01
1.000000000000000000e+02	7.616378473737830000e-01	8.295543913544620000e-01	8.499529674780340000e-01	6.016694160556230000e-01	8.523530284751400000e-01	6.396783484450330000e-01	8.835973463025320000e-01
2.000000000000000000e+02	8.615056987810160000e-01	8.480891648669360000e-01	8.682294808527260000e-01	7.411117493791040000e-01	9.389041472006520000e-01	7.395461998522660000e-01	9.834651977097650000e-01
3.000000000000000000e+02	9.902772607162270000e-01	9.653781930346940000e-01	9.717222970309080000e-01	9.408642005669170000e-01	1.039690320865540000e+00	8.683177617874770000e-01	1.112236759644980000e+00
4.000000000000000000e+02	9.445730037265040000e-01	8.538668711300510000e-01	9.672730014283980000e-01	8.428801081621520000e-01	1.038426843770430000e+00	8.226135047977550000e-01	1.066532502655250000e+00
5.000000000000000000e+02	8.789253628909170000e-01	8.471394251696220000e-01	9.020832805199030000e-01	7.635297456937020000e-01	9.570070385795210000e-01	6.653207577852040000e-01	8.071559298518250000e-01
6.000000000000000000e+02	9.092134980765720000e-01	8.919987976735600000e-01	9.277710831490240000e-01	8.052439028724690000e-01	9.851740803976770000e-01	6.933190111667260000e-01	7.663621217911210000e-01
7.000000000000000000e+02	9.585787854652360000e-01	9.184875907476770000e-01	9.728028755737380000e-01	8.682892839173810000e-01	1.030891464969580000e+00	7.276715616451330000e-01	7.663887792450240000e-01
8.000000000000000000e+02	9.365779865137060000e-01	8.985409951702660000e-01	9.497025006047220000e-01	8.520282520690320000e-01	1.007726476114320000e+00	5.438694771587890000e-01	7.663936955090830000e-01
9.000000000000000000e+02	8.868837808526850000e-01	8.519212145931850000e-01	9.090766056518210000e-01	7.869808951418260000e-01	9.682211054508180000e-01	5.445042713061280000e-01	7.653977284269230000e-01
1.000000000000000000e+03	8.570793065916060000e-01	8.305491303682300000e-01	8.882204701069110000e-01	7.569329788498420000e-01	9.349626175903970000e-01	5.443887047396640000e-01	7.657024860882930000e-01
1.100000000000000000e+03	8.140666070153020000e-01	7.875935212193760000e-01	8.455542980552010000e-01	7.141820160915220000e-01	8.916583751108950000e-01	5.442995045880890000e-01	7.657314928009170000e-01
1.200000000000000000e+03	7.713849752895880000e-01	7.450771852556590000e-01	8.029951827436320000e-01	6.782399340652240000e-01	8.460556522335790000e-01	5.453791847167450000e-01	5.501472608959280000e-01
1.300000000000000000e+03	7.732918164257080000e-01	7.447795284127560000e-01	8.028835056414870000e-01	6.823595480148020000e-01	8.458205500282430000e-01	5.444359790623390000e-01	5.505487050979190000e-01
1.400000000000000000e+03	8.117770913395220000e-01	7.876983437851650000e-01	8.427481021530610000e-01	7.243565868021520000e-01	8.809651772382150000e-01	5.441770156490150000e-01	7.659571593629020000e-01
1.500000000000000000e+03	8.531645655219060000e-01	8.316054173556120000e-01	8.866680241101160000e-01	7.612602132555650000e-01	9.235026663435090000e-01	5.432967158270380000e-01	7.674824023605770000e-01
1.600000000000000000e+03	8.896204540686720000e-01	8.744626336055330000e-01	9.267291974489970000e-01	7.991692715496670000e-01	9.586136329559810000e-01	5.437546605713660000e-01	7.673942249276390000e-01
1.700000000000000000e+03	8.740926278392280000e-01	8.523327881612910000e-01	9.046292908486490000e-01	7.774244541360860000e-01	9.477474324151480000e-01	5.435149550823280000e-01	7.674791455306420000e-01
1.800000000000000000e+03	9.151511844053140000e-01	8.957549296791530000e-01	9.478242592669330000e-01	8.121409395200720000e-01	9.905016534918820000e-01	5.439754742907390000e-01	7.672250102706480000e-01
1.900000000000000000e+03	8.805741958399650000e-01	8.560268988494850000e-01	9.076274533211110000e-01	7.800019673707150000e-01	9.546878771430120000e-01	5.437735909331680000e-01	7.667475524443890000e-01
2.000000000000000000e+03	8.259999908125520000e-01	8.090021881300950000e-01	8.415185261478880000e-01	7.327615933367150000e-01	8.982599180663140000e-01	5.456519112099710000e-01	7.639318997722200000e-01
2.100000000000000000e+03	8.277885950590370000e-01	8.086214226150840000e-01	8.408673798155420000e-01	7.324410127577340000e-01	9.022044621869550000e-01	5.445094856622850000e-01	7.642659946808640000e-01
2.200000000000000000e+03	8.794648850489950000e-01	8.729639675033250000e-01	9.054931516456020000e-01	7.766891928374350000e-01	9.560177510455980000e-01	5.441994960878330000e-01	7.642836114371280000e-01
2.300000000000000000e+03	8.322493833704080000e-01	8.082317997298400000e-01	8.653207396993770000e-01	7.265839296261250000e-01	9.171026380645280000e-01	5.437139544691430000e-01	7.653625053698740000e-01
2.400000000000000000e+03	8.700897002651830000e-01	8.473270711474000000e-01	9.074217467317600000e-01	7.592122674635270000e-01	9.587071423972960000e-01	5.392979157074300000e-01	7.678179027721930000e-01
2.500000000000000000e+03	9.053051433339260000e-01	8.711689596890390000e-01	9.491302444806220000e-01	8.011319889266460000e-01	9.903373296679300000e-01	5.374557023100480000e-01	7.675446940245170000e-01
2.600000000000000000e+03	8.981184305178000000e-01	8.675635044953670000e-01	9.483715991388580000e-01	7.802634229032830000e-01	9.890114673218200000e-01	5.362589593936040000e-01	7.673655494186820000e-01
2.700000000000000000e+03	9.019084666094220000e-01	8.677753703180010000e-01	9.290451266084120000e-01	7.988832324917850000e-01	9.848182071097220000e-01	5.358145196968670000e-01	7.662621156528570000e-01
2.800000000000000000e+03	9.525205945779560000e-01	9.318663474169250000e-01	9.679584520655350000e-01	8.658715618751450000e-01	1.022242606367060000e+00	7.266931753873400000e-01	7.578649135994900000e-01
2.900000000000000000e+03	9.546187764692220000e-01	9.132499748205160000e-01	9.865136506631470000e-01	8.703721738048930000e-01	1.027178121961780000e+00	7.266931753873400000e-01	7.578649135994900000e-01
3.000000000000000000e+03	9.635768893613030000e-01	9.353095518225390000e-01	9.868421040440260000e-01	8.836751180067150000e-01	1.027712798466020000e+00	7.266931753873400000e-01	7.578649135994900000e-01
3.100000000000000000e+03	9.636779280669460000e-01	9.356253795745540000e-01	9.867317302934550000e-01	8.945818532521790000e-01	1.023501980385430000e+00	7.567900260749330000e-01	7.578649135994900000e-01
3.200000000000000000e+03	9.591762999013730000e-01	9.353891214464320000e-01	9.865349312863590000e-01	8.815343949355190000e-01	1.023466873341230000e+00	7.567900260749330000e-01	7.578649135994900000e-01
3.300000000000000000e+03	9.569620306166970000e-01	9.354438740671570000e-01	9.865901181616440000e-01	8.728938649235540000e-01	1.023608733039370000e+00	7.567900260749330000e-01	7.578649135994900000e-01
3.400000000000000000e+03	9.461056662086350000e-01	9.354223763166670000e-01	9.647027402908300000e-01	8.630709979981330000e-01	1.010880429192830000e+00	7.567900260749330000e-01	7.578649135994900000e-01
3.500000000000000000e+03	9.480727107066040000e-01	9.349188388064620000e-01	9.644693671608240000e-01	8.541247417373920000e-01	1.024081340431170000e+00	7.567900260749330000e-01	7.578649135994900000e-01
3.600000000000000000e+03	9.500655524395560000e-01	9.161705947089900000e-01	9.860373808996670000e-01	8.426686516453900000e-01	1.034713090725580000e+00	7.266931753873400000e-01	7.578649135994900000e-01
3.700000000000000000e+03	9.411224875791840000e-01	8.942213914575390000e-01	9.825021983685770000e-01	8.328563548190610000e-01	1.030718567516930000e+00	7.266931753873400000e-01	7.578649135994900000e-01
3.800000000000000000e+03	9.257129002895600000e-01	8.721376488341890000e-01	9.821737449876980000e-01	8.091538147718150000e-01	1.017626341683180000e+00	7.165958142859060000e-01	7.578649135994900000e-01
3.900000000000000000e+03	9.299565554492400000e-01	8.905332739294550000e-01	9.822315997338200000e-01	8.135174605495920000e-01	1.017629860785150000e+00	7.165958142859060000e-01	7.578649135994900000e-01
4.000000000000000000e+03	9.125218797189190000e-01	8.689772344376360000e-01	9.601472057286300000e-01	7.953985455788660000e-01	1.004637462899640000e+00	7.155209267613490000e-01	7.578649135994900000e-01
4.100000000000000000e+03	9.081599869315390000e-01	8.689956300627310000e-01	9.385541578593400000e-01	8.076998158475570000e-01	9.936158480658990000e-01	7.256182878627830000e-01	7.578649135994900000e-01
4.200000000000000000e+03	9.062273379814790000e-01	8.875783135343460000e-01	9.419607881420430000e-01	7.881400867759240000e-01	9.977524737146180000e-01	6.912218870769630000e-01	7.578649135994900000e-01
4.300000000000000000e+03	9.083556152801010000e-01	8.875568157838550000e-01	9.416755473894260000e-01	7.913302911480250000e-01	1.008864548626140000e+00	6.955214371751910000e-01	7.578649135994900000e-01
4.400000000000000000e+03	9.106042798666640000e-01	8.691795863136840000e-01	9.633308548939130000e-01	7.891813135389660000e-01	1.019611014165970000e+00	6.955214371751910000e-01	7.578649135994900000e-01
4.500000000000000000e+03	9.105247379274230000e-01	8.691580885631930000e-01	9.633308548939130000e-01	7.940880310835560000e-01	1.014545213070930000e+00	6.955214371751910000e-01	7.578649135994900000e-01
4.600000000000000000e+03	9.192743217212570000e-01	8.691580885631930000e-01	9.850014558981000000e-01	7.989643878448100000e-01	1.025787971054690000e+00	6.955214371751910000e-01	7.578649135994900000e-01
4.700000000000000000e+03	9.059951629486350000e-01	8.505570094664830000e-01	9.629507510177040000e-01	7.971528887695960000e-01	1.003999857911000000e+00	7.256182878627830000e-01	7.578649135994900000e-01
4.800000000000000000e+03	9.060768547941370000e-01	8.505785072169740000e-01	9.661115996688170000e-01	7.825782510682460000e-01	1.009515138340050000e+00	7.155209267613490000e-01	7.578649135994900000e-01
4.900000000000000000e+03	9.104387482375770000e-01	8.505785072169740000e-01	9.663718062909870000e-01	7.871181786624740000e-01	1.012452499433760000e+00	7.155209267613490000e-01	7.578649135994900000e-01
5.000000000000000000e+03	9.152004997253420000e-01	8.505969028420690000e-01	9.914486033233160000e-01	7.653272657858050000e-01	1.034054221543560000e+00	7.112213766631210000e-01	7.578649135994900000e-01
}\SwitchShieldNormShield


==> figs/data/ShieldSwitching/obstacle_shield_switch_belief_support.tex <==
\pgfplotstableread{
0.000000000000000000e+00 7.604000244140625000e+02 6.677559695009582583e+02 8.530440793271667417e+02
1.000000000000000000e+02 9.930000000000000000e+02 9.003559450868957583e+02 1.000000000000000000e+03
2.000000000000000000e+02 9.904000244140625000e+02 8.977559695009582583e+02 1.000000000000000000e+03
3.000000000000000000e+02 9.924000244140625000e+02 8.997559695009582583e+02 1.000000000000000000e+03
4.000000000000000000e+02 9.922000122070312500e+02 8.995559572939270083e+02 1.000000000000000000e+03
5.000000000000000000e+02 9.456800170898437727e+02 9.003559450868957583e+02 1.000000000000000000e+03
6.000000000000000000e+02 9.921200073242187045e+02 9.894207046793437712e+02 9.948193099690936378e+02
7.000000000000000000e+02 9.921200073242187045e+02 9.003559450868957583e+02 1.000000000000000000e+03
8.000000000000000000e+02 9.456800170898437727e+02 9.003559450868957583e+02 1.000000000000000000e+03
9.000000000000000000e+02 9.921200073242187045e+02 1.779988583716316271e+02 1.000000000000000000e+03
1.000000000000000000e+03 7.684800048828125227e+02 1.412747624969852041e+02 1.000000000000000000e+03
1.100000000000000000e+03 6.755200073242187955e+02 3.263327658113329335e+02 1.000000000000000000e+03
1.200000000000000000e+03 5.827600097656250000e+02 3.085850034838398415e+02 1.000000000000000000e+03
1.300000000000000000e+03 5.730800048828125455e+02 2.041857764621808542e+02 1.000000000000000000e+03
1.400000000000000000e+03 4.826000000000000227e+02 1.397191717136529405e+02 1.000000000000000000e+03
1.500000000000000000e+03 4.913599914550781023e+02 8.494337535727936483e+00 9.742256453744282680e+02
1.600000000000000000e+03 4.902799987792968750e+02 8.125043425148533061e+00 9.724349541334452169e+02
1.700000000000000000e+03 5.347200012207031250e+02 -4.409182999854238005e+01 1.000000000000000000e+03
1.800000000000000000e+03 6.274399963378906477e+02 1.296750986014621958e+02 1.000000000000000000e+03
1.900000000000000000e+03 5.720399978637694858e+02 -2.257809908941342201e+02 1.000000000000000000e+03
2.000000000000000000e+03 4.813199966430664176e+02 -3.169920672840207203e+02 1.000000000000000000e+03
2.100000000000000000e+03 5.267599868774414062e+02 -3.369834808136911306e+02 1.000000000000000000e+03
2.200000000000000000e+03 5.279999893188476108e+02 -3.386781715384336167e+02 1.000000000000000000e+03
2.300000000000000000e+03 3.460799942016601562e+02 -7.406050063220916400e+02 1.000000000000000000e+03
2.400000000000000000e+03 4.371199890136718977e+02 -5.773448068317378556e+02 1.000000000000000000e+03
2.500000000000000000e+03 4.827599853515624773e+02 -5.127235324754459498e+02 1.000000000000000000e+03
2.600000000000000000e+03 3.937199890136718636e+02 -5.266751961621976079e+02 1.000000000000000000e+03
2.700000000000000000e+03 4.360799865722656250e+02 -6.545532248316810637e+02 1.000000000000000000e+03
2.800000000000000000e+03 6.160399841308593523e+02 -6.228483082979562369e+01 1.000000000000000000e+03
2.900000000000000000e+03 5.705999877929687045e+02 -2.088946421458886107e+02 1.000000000000000000e+03
3.000000000000000000e+03 6.591199951171875000e+02 -2.470730715440204222e+02 1.000000000000000000e+03
3.100000000000000000e+03 6.581999938964843295e+02 -2.512360706721506176e+02 1.000000000000000000e+03
3.200000000000000000e+03 6.140399963378906705e+02 -1.919334274922680379e+02 1.000000000000000000e+03
3.300000000000000000e+03 5.690399963378906705e+02 -2.130837578352550281e+02 1.000000000000000000e+03
3.400000000000000000e+03 6.138400024414062273e+02 -6.919242646450686607e+01 1.000000000000000000e+03
3.500000000000000000e+03 5.246400024414062955e+02 9.943333826806144771e+01 9.498466666147511432e+02
3.600000000000000000e+03 5.245200073242187955e+02 9.874459660462491684e+01 9.502954180438126741e+02
3.700000000000000000e+03 5.711600097656249773e+02 -9.820580015290681786e+01 1.000000000000000000e+03
3.800000000000000000e+03 5.717200073242187273e+02 -9.731261516987956384e+01 1.000000000000000000e+03
3.900000000000000000e+03 5.274800048828125227e+02 -2.185368999205207956e+02 1.000000000000000000e+03
4.000000000000000000e+03 5.732400024414062045e+02 -2.199956142485837063e+02 1.000000000000000000e+03
4.100000000000000000e+03 6.636800048828124545e+02 -2.855814502084149353e+01 1.000000000000000000e+03
4.200000000000000000e+03 5.719200073242187727e+02 6.574134128569238555e+01 1.000000000000000000e+03
4.300000000000000000e+03 5.729600097656250455e+02 6.754451055977182250e+01 1.000000000000000000e+03
4.400000000000000000e+03 6.629600097656250455e+02 3.336977574612043895e+02 9.922222620700456446e+02
4.500000000000000000e+03 6.173200073242187500e+02 2.865144334880798169e+02 9.481255811603576831e+02
4.600000000000000000e+03 5.274800048828125227e+02 1.013862805676294556e+02 9.535737291979955899e+02
4.700000000000000000e+03 5.280400024414062727e+02 1.019812912541839296e+02 9.540987136286286159e+02
4.800000000000000000e+03 5.614400024414062500e+02 8.694122628716127110e+01 1.000000000000000000e+03
4.900000000000000000e+03 4.710400024414062727e+02 1.393808745826902395e+01 9.281419174245435215e+02
5.000000000000000000e+03 5.629200073242187727e+02 -2.128133555535431469e+02 1.000000000000000000e+03
}\obstacleShieldSwitchOffSupp

\pgfplotstableread{
0.000000000000000000e+00 -1.990000000000000000e+02 -1.99000000000000000e+02 2.770200243317961508e+02
1.000000000000000000e+02 9.910000000000000000e+02 5.149799756682039060e+02 1.000000000000000000e+03
2.000000000000000000e+02 9.912000122070312500e+02 5.151799878752351560e+02 1.000000000000000000e+03
3.000000000000000000e+02 9.907999877929687500e+02 5.147799634611726560e+02 1.000000000000000000e+03
4.000000000000000000e+02 9.912000122070312500e+02 5.151799878752351560e+02 1.000000000000000000e+03
5.000000000000000000e+02 7.530400024414062727e+02 -6.750200705539822366e+02 1.000000000000000000e+03
6.000000000000000000e+02 9.910400024414062727e+02 9.905909761502762194e+02 9.914890287325363261e+02
7.000000000000000000e+02 9.910000000000000000e+02 9.904633109304979826e+02 9.915366890695020174e+02
8.000000000000000000e+02 9.908799926757812955e+02 9.902680729878157990e+02 9.914919123637467919e+02
9.000000000000000000e+02 9.910000000000000000e+02 9.901514200725287083e+02 9.918485799274712917e+02
1.000000000000000000e+03 9.910400024414062727e+02 9.900799438476562955e+02 9.920000610351562500e+02
1.100000000000000000e+03 9.910800048828125455e+02 9.901050607720218295e+02 9.920549489936032614e+02
1.200000000000000000e+03 9.910000122070312045e+02 9.897414171463956336e+02 9.922586072676667754e+02
1.300000000000000000e+03 9.910000122070312045e+02 9.897414171463956336e+02 9.922586072676667754e+02
1.400000000000000000e+03 9.907600097656250000e+02 9.893708973146930248e+02 9.921491222165569752e+02
1.500000000000000000e+03 9.908800048828125000e+02 9.889228726430212646e+02 9.928371371226037354e+02
1.600000000000000000e+03 9.908800048828125000e+02 9.889228726430212646e+02 9.928371371226037354e+02
1.700000000000000000e+03 9.910000000000000000e+02 9.891801074782637215e+02 9.928198925217362785e+02
1.800000000000000000e+03 9.911600097656249773e+02 9.894045666122265175e+02 9.929154529190234371e+02
1.900000000000000000e+03 9.913200073242187500e+02 9.902071723145830902e+02 9.924328423338544098e+02
2.000000000000000000e+03 9.911200073242187045e+02 9.906399780273436591e+02 9.916000366210937500e+02
2.100000000000000000e+03 9.909200073242187727e+02 9.897442477621767694e+02 9.920957668862607761e+02
2.200000000000000000e+03 9.908000122070312727e+02 9.894854814116482657e+02 9.921145430024142797e+02
2.300000000000000000e+03 9.908000122070312727e+02 9.894854814116482657e+02 9.921145430024142797e+02
2.400000000000000000e+03 9.906400146484375000e+02 9.892000122067724988e+02 9.920800170901025012e+02
2.500000000000000000e+03 9.907600097656250000e+02 9.889243895528911708e+02 9.925956299783588292e+02
2.600000000000000000e+03 9.909600097656250455e+02 9.892886299899728328e+02 9.926313895412772581e+02
2.700000000000000000e+03 9.909600097656250455e+02 9.892886299899728328e+02 9.926313895412772581e+02
2.800000000000000000e+03 9.907999999999999545e+02 9.892354223176628238e+02 9.923645776823370852e+02
2.900000000000000000e+03 9.910799926757812273e+02 9.895812277532068038e+02 9.925787575983556508e+02
3.000000000000000000e+03 9.910799926757812273e+02 9.895812277532068038e+02 9.925787575983556508e+02
3.100000000000000000e+03 9.910799926757812273e+02 9.895812277532068038e+02 9.925787575983556508e+02
3.200000000000000000e+03 9.913199829101562273e+02 9.901442345605428272e+02 9.924957312597696273e+02
3.300000000000000000e+03 9.915199829101562727e+02 9.910400268554687955e+02 9.919999389648437500e+02
3.400000000000000000e+03 9.913199829101562273e+02 9.901442345605428272e+02 9.924957312597696273e+02
3.500000000000000000e+03 9.911599853515624545e+02 9.899362249767549429e+02 9.923837457263699662e+02
3.600000000000000000e+03 9.910799804687500227e+02 9.897875504354611849e+02 9.923724105020388606e+02
3.700000000000000000e+03 9.909199829101562500e+02 9.898738547248896111e+02 9.919661110954228889e+02
3.800000000000000000e+03 9.907999877929687500e+02 9.904204913125352050e+02 9.911794842734022950e+02
3.900000000000000000e+03 9.909599975585937273e+02 9.902602406240450819e+02 9.916597544931423727e+02
4.000000000000000000e+03 9.909599975585937273e+02 9.902602406240450819e+02 9.916597544931423727e+02
4.100000000000000000e+03 9.909199951171874545e+02 9.901060658439439521e+02 9.917339243904309569e+02
4.200000000000000000e+03 9.908400024414062273e+02 9.898077072307853541e+02 9.918722976520271004e+02
4.300000000000000000e+03 9.908800048828125000e+02 9.897671501273904369e+02 9.919928596382345631e+02
4.400000000000000000e+03 9.907599975585937955e+02 9.899640087112571791e+02 9.915559864059304118e+02
4.500000000000000000e+03 9.907599975585937955e+02 9.899640087112571791e+02 9.915559864059304118e+02
4.600000000000000000e+03 9.910000000000000000e+02 9.895801625167970315e+02 9.924198374832029685e+02
4.700000000000000000e+03 9.910000000000000000e+02 9.895801625167970315e+02 9.924198374832029685e+02
4.800000000000000000e+03 9.909199951171874545e+02 9.895205911557653735e+02 9.923193990786095355e+02
4.900000000000000000e+03 9.910400024414062727e+02 9.895508539972159952e+02 9.925291508855965503e+02
5.000000000000000000e+03 9.911600097656249773e+02 9.896708613214346997e+02 9.926491582098152548e+02
}\obstacleShieldDecayedSwitchSupp

==> figs/data/VariableLength/Length100.tex <==
\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00
1.000000000000000000e+02 0.000000000000000000e+00
2.000000000000000000e+02 7.000000000000000000e+00
3.000000000000000000e+02 1.000000000000000000e+01
4.000000000000000000e+02 1.000000000000000000e+01
5.000000000000000000e+02 6.799999999999999822e+00
6.000000000000000000e+02 7.400000000000000355e+00
7.000000000000000000e+02 9.000000000000000000e+00
8.000000000000000000e+02 9.000000000000000000e+00
9.000000000000000000e+02 8.800000000000000711e+00
1.000000000000000000e+03 8.400000000000000355e+00
1.100000000000000000e+03 8.199999999999999289e+00
1.200000000000000000e+03 8.400000000000000355e+00
1.300000000000000000e+03 9.000000000000000000e+00
1.400000000000000000e+03 9.199999999999999289e+00
1.500000000000000000e+03 9.400000000000000355e+00
1.600000000000000000e+03 9.400000000000000355e+00
1.700000000000000000e+03 9.400000000000000355e+00
1.800000000000000000e+03 9.199999999999999289e+00
1.900000000000000000e+03 8.599999999999999645e+00
2.000000000000000000e+03 8.599999999999999645e+00
2.100000000000000000e+03 8.599999999999999645e+00
2.200000000000000000e+03 8.800000000000000711e+00
2.300000000000000000e+03 8.599999999999999645e+00
2.400000000000000000e+03 9.199999999999999289e+00
2.500000000000000000e+03 9.400000000000000355e+00
2.600000000000000000e+03 9.599999999999999645e+00
2.700000000000000000e+03 9.400000000000000355e+00
2.800000000000000000e+03 9.199999999999999289e+00
2.900000000000000000e+03 8.800000000000000711e+00
3.000000000000000000e+03 8.400000000000000355e+00
3.100000000000000000e+03 8.199999999999999289e+00
3.200000000000000000e+03 8.400000000000000355e+00
3.300000000000000000e+03 8.599999999999999645e+00
3.400000000000000000e+03 8.400000000000000355e+00
3.500000000000000000e+03 8.800000000000000711e+00
3.600000000000000000e+03 8.800000000000000711e+00
3.700000000000000000e+03 8.599999999999999645e+00
3.800000000000000000e+03 8.400000000000000355e+00
3.900000000000000000e+03 8.800000000000000711e+00
4.000000000000000000e+03 8.599999999999999645e+00
4.100000000000000000e+03 8.800000000000000711e+00
4.200000000000000000e+03 8.800000000000000711e+00
4.300000000000000000e+03 8.800000000000000711e+00
4.400000000000000000e+03 8.800000000000000711e+00
4.500000000000000000e+03 9.000000000000000000e+00
4.600000000000000000e+03 9.000000000000000000e+00
4.700000000000000000e+03 8.800000000000000711e+00
4.800000000000000000e+03 9.199999999999999289e+00
4.900000000000000000e+03 9.400000000000000355e+00
5.000000000000000000e+03 9.199999999999999289e+00
}\shieldvariablelenC

\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00
1.000000000000000000e+02 2.000000000000000000e+00
2.000000000000000000e+02 4.000000000000000000e+00
3.000000000000000000e+02 4.000000000000000000e+00
4.000000000000000000e+02 2.000000000000000000e+00
5.000000000000000000e+02 2.399999999999999911e+00
6.000000000000000000e+02 3.799999999999999822e+00
7.000000000000000000e+02 3.799999999999999822e+00
8.000000000000000000e+02 3.600000000000000089e+00
9.000000000000000000e+02 3.600000000000000089e+00
1.000000000000000000e+03 3.600000000000000089e+00
1.100000000000000000e+03 3.399999999999999911e+00
1.200000000000000000e+03 3.600000000000000089e+00
1.300000000000000000e+03 3.799999999999999822e+00
1.400000000000000000e+03 3.200000000000000178e+00
1.500000000000000000e+03 2.799999999999999822e+00
1.600000000000000000e+03 2.399999999999999911e+00
1.700000000000000000e+03 2.600000000000000089e+00
1.800000000000000000e+03 2.200000000000000178e+00
1.900000000000000000e+03 2.200000000000000178e+00
2.000000000000000000e+03 3.000000000000000000e+00
2.100000000000000000e+03 2.600000000000000089e+00
2.200000000000000000e+03 2.600000000000000089e+00
2.300000000000000000e+03 2.600000000000000089e+00
2.400000000000000000e+03 2.799999999999999822e+00
2.500000000000000000e+03 3.000000000000000000e+00
2.600000000000000000e+03 2.799999999999999822e+00
2.700000000000000000e+03 2.600000000000000089e+00
2.800000000000000000e+03 2.600000000000000089e+00
2.900000000000000000e+03 3.000000000000000000e+00
3.000000000000000000e+03 3.000000000000000000e+00
3.100000000000000000e+03 3.600000000000000089e+00
3.200000000000000000e+03 3.600000000000000089e+00
3.300000000000000000e+03 4.799999999999999822e+00
3.400000000000000000e+03 4.400000000000000355e+00
3.500000000000000000e+03 3.799999999999999822e+00
3.600000000000000000e+03 3.399999999999999911e+00
3.700000000000000000e+03 3.399999999999999911e+00
3.800000000000000000e+03 2.399999999999999911e+00
3.900000000000000000e+03 2.200000000000000178e+00
4.000000000000000000e+03 2.600000000000000089e+00
4.100000000000000000e+03 2.799999999999999822e+00
4.200000000000000000e+03 2.399999999999999911e+00
4.300000000000000000e+03 2.799999999999999822e+00
4.400000000000000000e+03 3.399999999999999911e+00
4.500000000000000000e+03 3.000000000000000000e+00
4.600000000000000000e+03 2.600000000000000089e+00
4.700000000000000000e+03 2.799999999999999822e+00
4.800000000000000000e+03 2.000000000000000000e+00
4.900000000000000000e+03 1.800000000000000044e+00
5.000000000000000000e+03 1.600000000000000089e+00
}\noshieldvariablelenC

==> figs/data/VariableLength/Length13.tex <==
\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
5.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
6.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
7.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
8.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
9.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.000000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.100000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.200000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.300000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.400000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.500000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.600000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.700000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.800000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.900000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.000000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.100000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.200000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.300000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.400000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.500000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.600000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.700000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.800000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.900000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.000000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.100000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.200000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.300000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.400000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.500000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.600000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.700000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.800000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.900000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.000000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.100000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.200000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.300000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.400000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.500000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.600000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.700000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.800000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.900000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
5.000000000000000000e+03 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00 
}\shieldvariablelenXIII

\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
1.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
2.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
3.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
4.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
5.000000000000000000e+02 0.000000000000000000e+00 0.000000000000000000e+00 0.000000000000000000e+00
6.000000000000000000e+02 5.999999999999999778e-01 1.799999999999999822e+00 -5.999999999999999778e-01
7.000000000000000000e+02 1.000000000000000000e+00 2.264911064067351987e+00 -2.649110640673517647e-01
8.000000000000000000e+02 2.799999999999999822e+00 6.110589071449370024e+00 -5.105890714493699356e-01
9.000000000000000000e+02 3.000000000000000000e+00 6.162277660168379967e+00 -1.622776601683795228e-01
1.000000000000000000e+03 3.799999999999999822e+00 6.585677655436823486e+00 1.014322344563176159e+00
1.100000000000000000e+03 4.200000000000000178e+00 6.985677655436823841e+00 1.414322344563176070e+00
1.200000000000000000e+03 4.400000000000000355e+00 7.053299832284320559e+00 1.746700167715680152e+00
1.300000000000000000e+03 3.799999999999999822e+00 5.520465053408525335e+00 2.079534946591474309e+00
1.400000000000000000e+03 4.599999999999999645e+00 5.619803902718556898e+00 3.580196097281442391e+00
1.500000000000000000e+03 4.000000000000000000e+00 5.788854381999831489e+00 2.211145618000168511e+00
1.600000000000000000e+03 3.399999999999999911e+00 5.254723699099140610e+00 1.545276300900859212e+00
1.700000000000000000e+03 2.799999999999999822e+00 5.115167380558045096e+00 4.848326194419545487e-01
1.800000000000000000e+03 2.000000000000000000e+00 3.673320053068151125e+00 3.266799469318488747e-01
1.900000000000000000e+03 1.000000000000000000e+00 1.894427190999915744e+00 1.055728090000841446e-01
2.000000000000000000e+03 1.600000000000000089e+00 3.096662954709576532e+00 1.033370452904234238e-01
2.100000000000000000e+03 1.399999999999999911e+00 2.896662954709576354e+00 -9.666295470957653180e-02
2.200000000000000000e+03 2.000000000000000000e+00 3.414213562373094923e+00 5.857864376269048545e-01
2.300000000000000000e+03 2.200000000000000178e+00 3.669693845669907084e+00 7.303061543300932712e-01
2.400000000000000000e+03 3.000000000000000000e+00 4.095445115010331705e+00 1.904554884989667851e+00
2.500000000000000000e+03 2.399999999999999911e+00 3.599999999999999645e+00 1.199999999999999956e+00
2.600000000000000000e+03 3.000000000000000000e+00 4.095445115010331705e+00 1.904554884989667851e+00
2.700000000000000000e+03 3.000000000000000000e+00 4.095445115010331705e+00 1.904554884989667851e+00
2.800000000000000000e+03 3.000000000000000000e+00 4.095445115010331705e+00 1.904554884989667851e+00
2.900000000000000000e+03 3.000000000000000000e+00 4.095445115010331705e+00 1.904554884989667851e+00
3.000000000000000000e+03 3.399999999999999911e+00 3.889897948556635399e+00 2.910102051443364424e+00
3.100000000000000000e+03 2.799999999999999822e+00 3.779795897113270797e+00 1.820204102886728625e+00
3.200000000000000000e+03 2.600000000000000089e+00 3.619803902718556898e+00 1.580196097281443057e+00
3.300000000000000000e+03 3.200000000000000178e+00 4.920465053408525691e+00 1.479534946591474887e+00
3.400000000000000000e+03 2.799999999999999822e+00 4.520465053408525335e+00 1.079534946591474531e+00
3.500000000000000000e+03 2.600000000000000089e+00 4.343559577416269413e+00 8.564404225837307649e-01
3.600000000000000000e+03 3.200000000000000178e+00 4.800000000000000711e+00 1.600000000000000089e+00
3.700000000000000000e+03 3.399999999999999911e+00 4.896662954709576354e+00 1.903337045290423468e+00
3.800000000000000000e+03 3.200000000000000178e+00 4.366190378969060149e+00 2.033809621030940207e+00
3.900000000000000000e+03 3.600000000000000089e+00 4.619803902718556898e+00 2.580196097281443279e+00
4.000000000000000000e+03 4.000000000000000000e+00 4.632455532033675993e+00 3.367544467966324007e+00
4.100000000000000000e+03 3.799999999999999822e+00 4.548331477354787822e+00 3.051668522645211823e+00
4.200000000000000000e+03 3.200000000000000178e+00 4.920465053408525691e+00 1.479534946591474887e+00
4.300000000000000000e+03 3.000000000000000000e+00 4.549193338482966809e+00 1.450806661517033191e+00
4.400000000000000000e+03 3.000000000000000000e+00 4.549193338482966809e+00 1.450806661517033191e+00
4.500000000000000000e+03 2.799999999999999822e+00 4.269693845669906729e+00 1.330306154330092694e+00
4.600000000000000000e+03 2.799999999999999822e+00 4.269693845669906729e+00 1.330306154330092916e+00
4.700000000000000000e+03 3.200000000000000178e+00 3.948331477354788177e+00 2.451668522645212178e+00
4.800000000000000000e+03 2.799999999999999822e+00 3.548331477354787822e+00 2.051668522645211823e+00
4.900000000000000000e+03 2.399999999999999911e+00 2.889897948556635399e+00 1.910102051443364424e+00
5.000000000000000000e+03 1.800000000000000044e+00 2.779795897113271241e+00 8.202041028867287364e-01
}\noshieldvariablelenXIII

==> figs/data/VariableLength/Length150.tex <==
\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00
1.000000000000000000e+02 0.000000000000000000e+00
2.000000000000000000e+02 1.000000000000000000e+01
3.000000000000000000e+02 9.000000000000000000e+00
4.000000000000000000e+02 1.000000000000000000e+01
5.000000000000000000e+02 5.799999999999999822e+00
6.000000000000000000e+02 7.799999999999999822e+00
7.000000000000000000e+02 9.800000000000000711e+00
8.000000000000000000e+02 9.599999999999999645e+00
9.000000000000000000e+02 9.800000000000000711e+00
1.000000000000000000e+03 9.800000000000000711e+00
1.100000000000000000e+03 9.800000000000000711e+00
1.200000000000000000e+03 9.599999999999999645e+00
1.300000000000000000e+03 9.800000000000000711e+00
1.400000000000000000e+03 9.800000000000000711e+00
1.500000000000000000e+03 9.800000000000000711e+00
1.600000000000000000e+03 9.800000000000000711e+00
1.700000000000000000e+03 1.000000000000000000e+01
1.800000000000000000e+03 9.800000000000000711e+00
1.900000000000000000e+03 9.800000000000000711e+00
2.000000000000000000e+03 9.599999999999999645e+00
2.100000000000000000e+03 9.599999999999999645e+00
2.200000000000000000e+03 9.599999999999999645e+00
2.300000000000000000e+03 9.800000000000000711e+00
2.400000000000000000e+03 9.800000000000000711e+00
2.500000000000000000e+03 1.000000000000000000e+01
2.600000000000000000e+03 1.000000000000000000e+01
2.700000000000000000e+03 9.800000000000000711e+00
2.800000000000000000e+03 9.800000000000000711e+00
2.900000000000000000e+03 9.800000000000000711e+00
3.000000000000000000e+03 9.800000000000000711e+00
3.100000000000000000e+03 9.800000000000000711e+00
3.200000000000000000e+03 1.000000000000000000e+01
3.300000000000000000e+03 1.000000000000000000e+01
3.400000000000000000e+03 1.000000000000000000e+01
3.500000000000000000e+03 1.000000000000000000e+01
3.600000000000000000e+03 1.000000000000000000e+01
3.700000000000000000e+03 1.000000000000000000e+01
3.800000000000000000e+03 1.000000000000000000e+01
3.900000000000000000e+03 1.000000000000000000e+01
4.000000000000000000e+03 1.000000000000000000e+01
4.100000000000000000e+03 1.000000000000000000e+01
4.200000000000000000e+03 1.000000000000000000e+01
4.300000000000000000e+03 1.000000000000000000e+01
4.400000000000000000e+03 1.000000000000000000e+01
4.500000000000000000e+03 9.800000000000000711e+00
4.600000000000000000e+03 9.800000000000000711e+00
4.700000000000000000e+03 9.800000000000000711e+00
4.800000000000000000e+03 9.800000000000000711e+00
4.900000000000000000e+03 9.800000000000000711e+00
5.000000000000000000e+03 1.000000000000000000e+01
}\shieldvariablelenCL

\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00
1.000000000000000000e+02 0.000000000000000000e+00
2.000000000000000000e+02 5.000000000000000000e+00
3.000000000000000000e+02 8.000000000000000000e+00
4.000000000000000000e+02 7.000000000000000000e+00
5.000000000000000000e+02 4.000000000000000000e+00
6.000000000000000000e+02 5.799999999999999822e+00
7.000000000000000000e+02 7.400000000000000355e+00
8.000000000000000000e+02 8.199999999999999289e+00
9.000000000000000000e+02 7.400000000000000355e+00
1.000000000000000000e+03 7.000000000000000000e+00
1.100000000000000000e+03 6.599999999999999645e+00
1.200000000000000000e+03 6.599999999999999645e+00
1.300000000000000000e+03 6.200000000000000178e+00
1.400000000000000000e+03 7.000000000000000000e+00
1.500000000000000000e+03 7.599999999999999645e+00
1.600000000000000000e+03 7.799999999999999822e+00
1.700000000000000000e+03 8.000000000000000000e+00
1.800000000000000000e+03 8.199999999999999289e+00
1.900000000000000000e+03 8.199999999999999289e+00
2.000000000000000000e+03 8.199999999999999289e+00
2.100000000000000000e+03 8.599999999999999645e+00
2.200000000000000000e+03 8.400000000000000355e+00
2.300000000000000000e+03 8.400000000000000355e+00
2.400000000000000000e+03 8.000000000000000000e+00
2.500000000000000000e+03 8.000000000000000000e+00
2.600000000000000000e+03 7.799999999999999822e+00
2.700000000000000000e+03 7.200000000000000178e+00
2.800000000000000000e+03 7.200000000000000178e+00
2.900000000000000000e+03 7.599999999999999645e+00
3.000000000000000000e+03 7.799999999999999822e+00
3.100000000000000000e+03 7.200000000000000178e+00
3.200000000000000000e+03 7.400000000000000355e+00
3.300000000000000000e+03 7.599999999999999645e+00
3.400000000000000000e+03 7.599999999999999645e+00
3.500000000000000000e+03 7.599999999999999645e+00
3.600000000000000000e+03 7.799999999999999822e+00
3.700000000000000000e+03 8.199999999999999289e+00
3.800000000000000000e+03 7.799999999999999822e+00
3.900000000000000000e+03 7.400000000000000355e+00
4.000000000000000000e+03 7.400000000000000355e+00
4.100000000000000000e+03 7.400000000000000355e+00
4.200000000000000000e+03 7.400000000000000355e+00
4.300000000000000000e+03 7.799999999999999822e+00
4.400000000000000000e+03 8.000000000000000000e+00
4.500000000000000000e+03 8.000000000000000000e+00
4.600000000000000000e+03 8.000000000000000000e+00
4.700000000000000000e+03 8.000000000000000000e+00
4.800000000000000000e+03 8.199999999999999289e+00
4.900000000000000000e+03 7.799999999999999822e+00
5.000000000000000000e+03 7.400000000000000355e+00
}\noshieldvariablelenCL

==> figs/data/VariableLength/Length25.tex <==
\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00 1.199999999999999956e+00 -1.199999999999999956e+00
1.000000000000000000e+02 0.000000000000000000e+00 1.199999999999999956e+00 -1.199999999999999956e+00
2.000000000000000000e+02 0.000000000000000000e+00 1.199999999999999956e+00 -1.199999999999999956e+00
3.000000000000000000e+02 0.000000000000000000e+00 1.199999999999999956e+00 -1.199999999999999956e+00
4.000000000000000000e+02 3.000000000000000000e+00 4.200000000000000178e+00 1.800000000000000044e+00
5.000000000000000000e+02 5.999999999999999778e-01 1.799999999999999822e+00 -5.999999999999999778e-01
6.000000000000000000e+02 1.199999999999999956e+00 2.669693845669907084e+00 -2.696938456699069508e-01
7.000000000000000000e+02 2.000000000000000000e+00 3.673320053068151125e+00 3.266799469318488747e-01
8.000000000000000000e+02 2.799999999999999822e+00 4.269693845669906729e+00 1.330306154330092916e+00
9.000000000000000000e+02 3.799999999999999822e+00 4.548331477354787822e+00 3.051668522645211823e+00
1.000000000000000000e+03 4.000000000000000000e+00 4.632455532033675993e+00 3.367544467966324007e+00
1.100000000000000000e+03 3.799999999999999822e+00 4.779795897113270797e+00 2.820204102886728847e+00
1.200000000000000000e+03 3.799999999999999822e+00 4.779795897113270797e+00 2.820204102886728847e+00
1.300000000000000000e+03 3.600000000000000089e+00 4.619803902718556898e+00 2.580196097281443279e+00
1.400000000000000000e+03 3.200000000000000178e+00 3.948331477354788177e+00 2.451668522645212178e+00
1.500000000000000000e+03 3.600000000000000089e+00 4.956465996625054160e+00 2.243534003374946018e+00
1.600000000000000000e+03 4.000000000000000000e+00 5.095445115010331705e+00 2.904554884989667851e+00
1.700000000000000000e+03 4.000000000000000000e+00 5.095445115010331705e+00 2.904554884989667851e+00
1.800000000000000000e+03 4.000000000000000000e+00 5.095445115010331705e+00 2.904554884989667851e+00
1.900000000000000000e+03 4.000000000000000000e+00 5.095445115010331705e+00 2.904554884989667851e+00
2.000000000000000000e+03 3.399999999999999911e+00 3.889897948556635399e+00 2.910102051443364424e+00
2.100000000000000000e+03 3.399999999999999911e+00 3.889897948556635399e+00 2.910102051443364424e+00
2.200000000000000000e+03 3.600000000000000089e+00 4.400000000000000355e+00 2.799999999999999822e+00
2.300000000000000000e+03 3.799999999999999822e+00 4.548331477354787822e+00 3.051668522645211823e+00
2.400000000000000000e+03 3.799999999999999822e+00 4.548331477354787822e+00 3.051668522645211823e+00
2.500000000000000000e+03 3.799999999999999822e+00 4.548331477354787822e+00 3.051668522645211823e+00
2.600000000000000000e+03 3.799999999999999822e+00 4.548331477354787822e+00 3.051668522645211823e+00
2.700000000000000000e+03 3.600000000000000089e+00 4.089897948556635576e+00 3.110102051443364601e+00
2.800000000000000000e+03 3.399999999999999911e+00 3.889897948556635399e+00 2.910102051443364424e+00
2.900000000000000000e+03 3.399999999999999911e+00 3.889897948556635399e+00 2.910102051443364424e+00
3.000000000000000000e+03 4.200000000000000178e+00 5.669693845669907084e+00 2.730306154330093271e+00
3.100000000000000000e+03 4.400000000000000355e+00 5.896662954709576354e+00 2.903337045290423912e+00
3.200000000000000000e+03 4.799999999999999822e+00 6.400000000000000355e+00 3.199999999999999734e+00
3.300000000000000000e+03 5.200000000000000178e+00 6.526649916142160279e+00 3.873350083857840076e+00
3.400000000000000000e+03 5.200000000000000178e+00 6.526649916142160279e+00 3.873350083857840076e+00
3.500000000000000000e+03 4.799999999999999822e+00 5.779795897113270797e+00 3.820204102886728847e+00
3.600000000000000000e+03 4.000000000000000000e+00 5.788854381999831489e+00 2.211145618000168511e+00
3.700000000000000000e+03 3.600000000000000089e+00 5.096662954709576532e+00 2.103337045290423646e+00
3.800000000000000000e+03 3.200000000000000178e+00 4.526649916142160279e+00 1.873350083857840076e+00
3.900000000000000000e+03 3.399999999999999911e+00 4.756465996625053094e+00 2.043534003374946284e+00
4.000000000000000000e+03 3.399999999999999911e+00 4.756465996625053982e+00 2.043534003374945840e+00
4.100000000000000000e+03 4.000000000000000000e+00 4.632455532033675993e+00 3.367544467966324007e+00
4.200000000000000000e+03 4.000000000000000000e+00 4.632455532033675993e+00 3.367544467966324007e+00
4.300000000000000000e+03 4.200000000000000178e+00 4.600000000000000533e+00 3.800000000000000266e+00
4.400000000000000000e+03 4.200000000000000178e+00 4.600000000000000533e+00 3.800000000000000266e+00
4.500000000000000000e+03 4.000000000000000000e+00 4.000000000000000000e+00 4.000000000000000000e+00
4.600000000000000000e+03 4.400000000000000355e+00 5.200000000000000178e+00 3.600000000000000533e+00
4.700000000000000000e+03 4.200000000000000178e+00 5.179795897113271153e+00 3.220204102886729203e+00
4.800000000000000000e+03 3.600000000000000089e+00 5.224807680927192166e+00 1.975192319072808012e+00
4.900000000000000000e+03 3.399999999999999911e+00 5.024807680927191988e+00 1.775192319072807834e+00
5.000000000000000000e+03 3.200000000000000178e+00 4.800000000000000711e+00 1.600000000000000089e+00
}\shieldvariablelenXXV

\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00 1.019803902718557032e+00 -1.019803902718557032e+00
1.000000000000000000e+02 1.000000000000000000e+00 2.019803902718557254e+00 -1.980390271855703155e-02
2.000000000000000000e+02 2.000000000000000000e+00 3.019803902718557254e+00 9.801960972814429685e-01
3.000000000000000000e+02 3.000000000000000000e+00 4.019803902718557254e+00 1.980196097281442968e+00
4.000000000000000000e+02 2.000000000000000000e+00 3.019803902718557254e+00 9.801960972814429685e-01
5.000000000000000000e+02 1.600000000000000089e+00 2.619803902718556898e+00 5.801960972814430573e-01
6.000000000000000000e+02 2.399999999999999911e+00 3.419803902718556721e+00 1.380196097281442880e+00
7.000000000000000000e+02 2.799999999999999822e+00 3.548331477354787822e+00 2.051668522645211823e+00
8.000000000000000000e+02 3.200000000000000178e+00 3.948331477354788177e+00 2.451668522645212178e+00
9.000000000000000000e+02 3.000000000000000000e+00 3.894427190999915744e+00 2.105572809000084256e+00
1.000000000000000000e+03 3.200000000000000178e+00 3.948331477354788177e+00 2.451668522645212178e+00
1.100000000000000000e+03 3.000000000000000000e+00 3.632455532033675993e+00 2.367544467966324007e+00
1.200000000000000000e+03 2.799999999999999822e+00 3.548331477354787822e+00 2.051668522645211823e+00
1.300000000000000000e+03 2.799999999999999822e+00 3.548331477354787822e+00 2.051668522645211823e+00
1.400000000000000000e+03 3.200000000000000178e+00 3.948331477354788177e+00 2.451668522645212178e+00
1.500000000000000000e+03 3.000000000000000000e+00 3.894427190999915744e+00 2.105572809000084256e+00
1.600000000000000000e+03 2.399999999999999911e+00 3.896662954709576354e+00 9.033370452904232462e-01
1.700000000000000000e+03 2.600000000000000089e+00 4.096662954709576532e+00 1.103337045290423646e+00
1.800000000000000000e+03 2.799999999999999822e+00 4.520465053408525335e+00 1.079534946591474531e+00
1.900000000000000000e+03 2.399999999999999911e+00 4.024807680927191988e+00 7.751923190728078339e-01
2.000000000000000000e+03 2.200000000000000178e+00 3.920465053408525691e+00 4.795349465914748865e-01
2.100000000000000000e+03 3.000000000000000000e+00 4.414213562373094923e+00 1.585786437626904855e+00
2.200000000000000000e+03 2.600000000000000089e+00 4.224807680927192166e+00 9.751923190728080115e-01
2.300000000000000000e+03 2.399999999999999911e+00 3.756465996625053538e+00 1.043534003374946284e+00
2.400000000000000000e+03 2.600000000000000089e+00 3.956465996625054160e+00 1.243534003374946240e+00
2.500000000000000000e+03 2.600000000000000089e+00 3.956465996625054160e+00 1.243534003374946240e+00
2.600000000000000000e+03 2.799999999999999822e+00 4.400000000000000355e+00 1.199999999999999734e+00
2.700000000000000000e+03 3.000000000000000000e+00 4.414213562373094923e+00 1.585786437626904855e+00
2.800000000000000000e+03 2.799999999999999822e+00 4.126649916142159924e+00 1.473350083857839721e+00
2.900000000000000000e+03 2.200000000000000178e+00 3.920465053408525691e+00 4.795349465914748865e-01
3.000000000000000000e+03 3.000000000000000000e+00 4.897366596101027980e+00 1.102633403898972464e+00
3.100000000000000000e+03 2.799999999999999822e+00 4.520465053408525335e+00 1.079534946591474531e+00
3.200000000000000000e+03 3.600000000000000089e+00 5.659126028197400515e+00 1.540873971802600106e+00
3.300000000000000000e+03 3.600000000000000089e+00 5.659126028197400515e+00 1.540873971802600106e+00
3.400000000000000000e+03 4.799999999999999822e+00 5.966190378969059793e+00 3.633809621030939851e+00
3.500000000000000000e+03 4.400000000000000355e+00 5.756465996625053982e+00 3.043534003374946728e+00
3.600000000000000000e+03 4.000000000000000000e+00 5.673320053068151125e+00 2.326679946931848875e+00
3.700000000000000000e+03 3.200000000000000178e+00 4.669693845669907084e+00 1.730306154330093271e+00
3.800000000000000000e+03 3.000000000000000000e+00 4.549193338482966809e+00 1.450806661517033191e+00
3.900000000000000000e+03 2.399999999999999911e+00 2.889897948556635399e+00 1.910102051443364424e+00
4.000000000000000000e+03 2.200000000000000178e+00 2.600000000000000089e+00 1.800000000000000266e+00
4.100000000000000000e+03 2.799999999999999822e+00 3.966190378969059793e+00 1.633809621030939851e+00
4.200000000000000000e+03 2.799999999999999822e+00 3.966190378969059793e+00 1.633809621030939851e+00
4.300000000000000000e+03 2.799999999999999822e+00 3.966190378969059793e+00 1.633809621030939851e+00
4.400000000000000000e+03 2.799999999999999822e+00 3.966190378969059793e+00 1.633809621030939851e+00
4.500000000000000000e+03 3.399999999999999911e+00 4.756465996625053982e+00 2.043534003374945840e+00
4.600000000000000000e+03 2.799999999999999822e+00 3.966190378969059793e+00 1.633809621030939851e+00
4.700000000000000000e+03 2.799999999999999822e+00 3.966190378969059793e+00 1.633809621030939851e+00
4.800000000000000000e+03 2.799999999999999822e+00 3.966190378969059793e+00 1.633809621030939851e+00
4.900000000000000000e+03 2.399999999999999911e+00 3.756465996625053982e+00 1.043534003374946062e+00
5.000000000000000000e+03 1.800000000000000044e+00 2.200000000000000178e+00 1.399999999999999911e+00
}\noshieldvariablelenXXV





==> figs/data/VariableLength/Length50.tex <==
\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00
1.000000000000000000e+02 0.000000000000000000e+00
2.000000000000000000e+02 5.000000000000000000e+00
3.000000000000000000e+02 8.000000000000000000e+00
4.000000000000000000e+02 4.000000000000000000e+00
5.000000000000000000e+02 3.399999999999999911e+00
6.000000000000000000e+02 5.000000000000000000e+00
7.000000000000000000e+02 6.599999999999999645e+00
8.000000000000000000e+02 7.400000000000000355e+00
9.000000000000000000e+02 7.400000000000000355e+00
1.000000000000000000e+03 8.000000000000000000e+00
1.100000000000000000e+03 7.599999999999999645e+00
1.200000000000000000e+03 7.799999999999999822e+00
1.300000000000000000e+03 7.799999999999999822e+00
1.400000000000000000e+03 7.200000000000000178e+00
1.500000000000000000e+03 7.000000000000000000e+00
1.600000000000000000e+03 7.000000000000000000e+00
1.700000000000000000e+03 7.200000000000000178e+00
1.800000000000000000e+03 6.599999999999999645e+00
1.900000000000000000e+03 7.200000000000000178e+00
2.000000000000000000e+03 7.799999999999999822e+00
2.100000000000000000e+03 7.799999999999999822e+00
2.200000000000000000e+03 7.400000000000000355e+00
2.300000000000000000e+03 8.000000000000000000e+00
2.400000000000000000e+03 8.199999999999999289e+00
2.500000000000000000e+03 7.000000000000000000e+00
2.600000000000000000e+03 6.799999999999999822e+00
2.700000000000000000e+03 6.400000000000000355e+00
2.800000000000000000e+03 6.000000000000000000e+00
2.900000000000000000e+03 5.000000000000000000e+00
3.000000000000000000e+03 5.599999999999999645e+00
3.100000000000000000e+03 6.400000000000000355e+00
3.200000000000000000e+03 7.000000000000000000e+00
3.300000000000000000e+03 7.000000000000000000e+00
3.400000000000000000e+03 7.599999999999999645e+00
3.500000000000000000e+03 8.000000000000000000e+00
3.600000000000000000e+03 8.000000000000000000e+00
3.700000000000000000e+03 7.799999999999999822e+00
3.800000000000000000e+03 7.400000000000000355e+00
3.900000000000000000e+03 8.000000000000000000e+00
4.000000000000000000e+03 8.199999999999999289e+00
4.100000000000000000e+03 7.799999999999999822e+00
4.200000000000000000e+03 7.799999999999999822e+00
4.300000000000000000e+03 8.199999999999999289e+00
4.400000000000000000e+03 7.599999999999999645e+00
4.500000000000000000e+03 7.400000000000000355e+00
4.600000000000000000e+03 7.200000000000000178e+00
4.700000000000000000e+03 6.599999999999999645e+00
4.800000000000000000e+03 6.000000000000000000e+00
4.900000000000000000e+03 6.400000000000000355e+00
5.000000000000000000e+03 6.000000000000000000e+00
}\shieldvariablelenL

\pgfplotstableread{
0.000000000000000000e+00 0.000000000000000000e+00
1.000000000000000000e+02 3.000000000000000000e+00
2.000000000000000000e+02 2.000000000000000000e+00
3.000000000000000000e+02 4.000000000000000000e+00
4.000000000000000000e+02 3.000000000000000000e+00
5.000000000000000000e+02 2.399999999999999911e+00
6.000000000000000000e+02 2.799999999999999822e+00
7.000000000000000000e+02 3.000000000000000000e+00
8.000000000000000000e+02 3.200000000000000178e+00
9.000000000000000000e+02 3.000000000000000000e+00
1.000000000000000000e+03 3.200000000000000178e+00
1.100000000000000000e+03 3.399999999999999911e+00
1.200000000000000000e+03 3.399999999999999911e+00
1.300000000000000000e+03 3.600000000000000089e+00
1.400000000000000000e+03 3.799999999999999822e+00
1.500000000000000000e+03 3.399999999999999911e+00
1.600000000000000000e+03 2.799999999999999822e+00
1.700000000000000000e+03 2.600000000000000089e+00
1.800000000000000000e+03 2.799999999999999822e+00
1.900000000000000000e+03 2.399999999999999911e+00
2.000000000000000000e+03 2.200000000000000178e+00
2.100000000000000000e+03 3.000000000000000000e+00
2.200000000000000000e+03 2.600000000000000089e+00
2.300000000000000000e+03 2.399999999999999911e+00
2.400000000000000000e+03 2.600000000000000089e+00
2.500000000000000000e+03 2.600000000000000089e+00
2.600000000000000000e+03 2.799999999999999822e+00
2.700000000000000000e+03 3.000000000000000000e+00
2.800000000000000000e+03 2.799999999999999822e+00
2.900000000000000000e+03 2.200000000000000178e+00
3.000000000000000000e+03 3.000000000000000000e+00
3.100000000000000000e+03 2.799999999999999822e+00
3.200000000000000000e+03 3.600000000000000089e+00
3.300000000000000000e+03 3.600000000000000089e+00
3.400000000000000000e+03 4.799999999999999822e+00
3.500000000000000000e+03 4.400000000000000355e+00
3.600000000000000000e+03 4.000000000000000000e+00
3.700000000000000000e+03 3.200000000000000178e+00
3.800000000000000000e+03 3.000000000000000000e+00
3.900000000000000000e+03 2.399999999999999911e+00
4.000000000000000000e+03 2.200000000000000178e+00
4.100000000000000000e+03 2.799999999999999822e+00
4.200000000000000000e+03 2.799999999999999822e+00
4.300000000000000000e+03 2.799999999999999822e+00
4.400000000000000000e+03 2.799999999999999822e+00
4.500000000000000000e+03 3.399999999999999911e+00
4.600000000000000000e+03 2.799999999999999822e+00
4.700000000000000000e+03 2.799999999999999822e+00
4.800000000000000000e+03 2.799999999999999822e+00
4.900000000000000000e+03 2.399999999999999911e+00
5.000000000000000000e+03 1.800000000000000044e+00
}\noshieldvariablelenL

==> figs/data/rocks3/noshield_ddqn_obs_valuation.tex <==
\addplot[dashed,blue] table {%

};


==> figs/data/rocks3/noshield_dqn_obs_valuation.tex <==
\addplot[dashed,blue] table {%
0.000000000000000000e+00 -1.008000000000000000e+03
1.000000000000000000e+03 -2.376000061035156250e+02
2.000000000000000000e+03 -2.603999938964843750e+02
3.000000000000000000e+03 -2.600000000000000000e+02
4.000000000000000000e+03 -2.607999877929687500e+02
5.000000000000000000e+03 -2.602000122070312500e+02
6.000000000000000000e+03 -2.603999938964843750e+02
7.000000000000000000e+03 -2.602000122070312500e+02
8.000000000000000000e+03 -2.597999877929687500e+02
9.000000000000000000e+03 -1.010200012207031250e+03
1.000000000000000000e+04 -2.593999938964843750e+02
};

==> figs/data/rocks3/noshield_ppo_obs_valuation.tex <==
\addplot[dashed,blue] table {%

};


==> figs/data/rocks3/noshield_reinforce_obs_valuation.tex <==
\addplot[dashed,blue] table {%

};


==> figs/data/rocks3/noshield_sac_obs_valuation.tex <==
\addplot[dashed,blue] table {%

};


==> figs/data/rocks3/shield_ddqn_obs_valuation.tex <==
\addplot[blue] table {%

};


==> figs/data/rocks3/shield_dqn_obs_valuation.tex <==
\addplot[blue] table {%
0.000000000000000000e+00 -2.603999938964843750e+02
1.000000000000000000e+03 -2.606000061035156250e+02
2.000000000000000000e+03 -2.602000122070312500e+02
3.000000000000000000e+03 -2.597999877929687500e+02
4.000000000000000000e+03 9.590000000000000000e+02
5.000000000000000000e+03 9.712000122070312500e+02
6.000000000000000000e+03 -2.603999938964843750e+02
7.000000000000000000e+03 -2.600000000000000000e+02
8.000000000000000000e+03 -2.596000061035156250e+02
9.000000000000000000e+03 9.587999877929687500e+02
1.000000000000000000e+04 9.592999877929687500e+02
};

==> figs/data/rocks3/shield_ppo_obs_valuation.tex <==
\addplot[blue] table {%

};


==> figs/data/rocks3/shield_reinforce_obs_valuation.tex <==
\addplot[blue] table {%

};


==> figs/data/rocks3/shield_sac_obs_valuation.tex <==
\addplot[blue] table {%

};


==> figs/domain_template.tex <==
\newcommand{\domaintemplate}[3]{
\begin{tikzpicture}
\begin{groupplot}[group style={group size=3 by 2,vertical sep=1.95cm,horizontal sep=1.35cm}]

% Refuel
\nextgroupplot[
xlabel = {Number of episodes},
xlabel style={yshift=0.15cm,xshift=-0.5cm},
ylabel = {Average Reward},
ylabel style={yshift=-0.35cm},
xmin=0,
xmax=5000,
width = 0.35*\textwidth,
height = \rlgraphheight,
scaled x ticks=base 10:-3,
xticklabel style={/pgf/number format/precision=2},
no markers,
legend cell align={left},
legend columns=3,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1.75,1.25)}, anchor=north, draw=none, /tikz/every even column/.append style={column sep=0.01cm}},
very thick]
\addplot +[mark=none,randomgray] coordinates {(0, 1.9) (5000, 1.9)};
\addlegendentry{Random Policy}
\addplot +[mark=none,randomgray,dashed,forget plot] coordinates {(0, 0.1) (5000, 0.1)};
\tubeplotindex{dashed,red,forget plot}{\fuelnoshieldREINFORCEObs}{6}{7}
\tubeplotindex{red}{\fuelshieldREINFORCEObs}{6}{7}
\addlegendentry{Observation}
\tubeplotindex{dashed,blue, forget plot}{\fuelnoshieldREINFORCESupp}{7}{6}
\tubeplotindex{blue}{\fuelshieldREINFORCESupp}{6}{7}
\addlegendentry{Belief Support}

% Evade
\nextgroupplot[
xlabel = {},
ylabel = {},
xmin=0,
xmax=5000,
ymin= 0,
% % 	ymax= 1.0,
% 	label style={font=\small},
% 	tick label style={font=\small},
width = 0.35*\textwidth,
height = \rlgraphheight,
scaled x ticks=base 10:-3,
xticklabel style={/pgf/number format/precision=2},
no markers,
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.05,0.90)}, anchor=north, draw=white!80!black, /tikz/every even column/.append style={column sep=0.01cm}},
very thick]
\addplot +[mark=none,randomgray] coordinates {(0, 0.8) (5000, 0.8)};
\addplot +[mark=none,randomgray,dashed,forget plot] coordinates {(0, 0.5) (5000, 0.5)};
\tubeplotindex{dashed,red,forget plot}{\evadenoshieldREINFORCEObs}{2}{3}
\tubeplotindex{red}{\evadeshieldREINFORCEObs}{2}{3}
\tubeplotindex{dashed,blue,forget plot}{\evadenoshieldREINFORCESupp}{2}{3}
\tubeplotindex{blue}{\evadeshieldREINFORCESupp}{2}{3}

% Rocks
\nextgroupplot[
xlabel = {},
ylabel = {},
ylabel style={yshift=-0.5em},
xmin=0,
xmax=5000,
width = 0.35*\textwidth,
height = \rlgraphheight,
scaled x ticks=base 10:-3,
xticklabel style={/pgf/number format/precision=2},
no markers]
\addplot +[mark=none,randomgray] coordinates {(0,11.7) (5000, 11.7)};
\addplot +[mark=none,randomgray,dashed,forget plot] coordinates {(0,8) (5000, 8)};
\tubeplotindex{dashed,red, forget plot}{\rocksnoshieldREINFORCEObs}{2}{3}
 \tubeplotindex{dashed,blue, forget plot]}{\rocksnoshieldREINFORCESupp}{2}{3}
\tubeplotindex{blue,forget plot}{\rocksshieldREINFORCESupp}{2}{3}
\tubeplotindex{red,forget plot}{\rocksshieldREINFORCEObs}{2}{3}

% Intercept
\nextgroupplot[
xlabel = {Number of episodes},
xlabel style={yshift=0.15cm,xshift=-0.5cm},
ylabel = {},
ylabel style={yshift=0.35cm},
xmin=0,
xmax=5000,
width = 0.35*\textwidth,
height = \rlgraphheight,
scaled x ticks=base 10:-3,
xticklabel style={/pgf/number format/precision=2},
no markers,
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,1.15)}, anchor=north, draw=white!80!black, /tikz/every even column/.append style={column sep=0.01cm}},
very thick]
\addplot +[mark=none,randomgray] coordinates {(0, 11) (5000, 11)};
\addplot +[mark=none,randomgray,dashed,forget plot] coordinates {(0, 5) (5000, 5)};
\tubeplotindex{dashed,red,forget plot}{\interceptnoshieldREINFORCEObs}{2}{3}
\tubeplotindex{red}{\interceptshieldREINFORCEObs}{2}{3}
\tubeplotindex{dashed,blue,forget plot}{\interceptnoshieldREINFORCESupp}{2}{3}
\tubeplotindex{blue}{\interceptshieldREINFORCESupp}{2}{3}


% Avoid
\nextgroupplot[
xlabel = {},
ylabel = {},
ylabel style={yshift=-0.35cm},
xmin=0,
xmax=5000,
width = 0.35*\textwidth,
height = \rlgraphheight,
scaled x ticks=base 10:-3,
xticklabel style={/pgf/number format/precision=2},
no markers,
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,1.15)}, anchor=north, draw=white!80!black, /tikz/every even column/.append style={column sep=0.01cm}},
very thick]
\addplot +[mark=none,randomgray] coordinates {(0, -100.30) (5000, -100.30)};
\addplot +[mark=none,randomgray,dashed,forget plot] coordinates {(0, -380) (5000, -380)};


\tubeplotindex{dashed,red,forget plot}{\avoidnoshieldREINFORCEObs}{2}{3}
\tubeplotindex{red}{\avoidshieldREINFORCEObs}{2}{3}
\tubeplotindex{dashed,blue,forget plot}{\avoidnoshieldREINFORCESupp}{6}{7}
\tubeplotindex{blue}{\avoidshieldREINFORCESupp}{2}{4}


% Obstacle
\nextgroupplot[
xlabel = {},
ylabel = {},
xmin=0,
xmax=5000,
width = 0.35*\textwidth,
height = \rlgraphheight,
scaled x ticks=base 10:-3,
xticklabel style={/pgf/number format/precision=2},
no markers,
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,1.15)}, anchor=north, draw=white!80!black, /tikz/every even column/.append style={column sep=0.01cm}},
very thick]

\addplot +[mark=none,randomgray] coordinates {(0,136.84 ) (5000, 136.84)};
\addplot +[mark=none,randomgray,dashed,forget plot] coordinates {(0,-951.35) (5000, -951.35)};
\tubeplotindex{dashed,red,forget plot}{\obstaclenoshieldREINFORCEObs}{2}{3}
\tubeplotindex{red}{\obstacleshieldREINFORCEObs}{4}{5}
\tubeplotindex{dashed,blue,forget plot}{\obstaclenoshieldREINFORCESupp}{2}{3}
\tubeplotindex{blue}{\obstacleshieldREINFORCESupp}{2}{3}

\end{groupplot}
\node[text width=6cm,align=center,anchor=north] at ([yshift=-7.5mm]group c1r1.south) {\subcaption{\domain{Refuel} (N=6, Energy=8) \label{#3-fig:refuel}}};
\node[text width=6cm,align=center,anchor=north] at ([yshift=-7.5mm]group c2r1.south) {\subcaption{\domain{Evade} (N=6, Radius=2) \label{#3-fig:evade}}};
\node[text width=6cm,align=center,anchor=north] at ([yshift=-7.5mm]group c3r1.south) {\subcaption{\domain{Rocks} (N=4) \label{#3-fig:rocks}}};
\node[text width=6cm,align=center,anchor=north] at ([yshift=-7.5mm]group c1r2.south){\subcaption{\domain{Intercept} (N=7, Radius=1) \label{#3-fig:intercept}}};
\node[text width=6cm,align=center,anchor=north] at ([yshift=-7.5mm]group c2r2.south){\subcaption{\domain{Avoid} (N=6, Radius=3) \label{#3-fig:avoid}}};
\node[text width=6cm,align=center,anchor=north] at ([yshift=-7.5mm]group c3r2.south){\subcaption{\domain{Obstacle} (N=6) \label{#3-fig:obstacle}}};
\end{tikzpicture}
{#2}
\label{#3}
}

\caption{REINFORCE {with} (solid) and {without} (dashed) a shield. The red lines show when the RL agent is trained using only observations from the environment, and the blue lines indicate when the RL agent is trained using the state estimator. The gray lines are the rewards, averaged over multiple evaluations, obtained via a policy that randomly selects from available actions.}
\label{fig:test}

==> related.tex <==
%\section{Related work}

\input{figs/data/VariableLength/Length13}
\input{figs/data/VariableLength/Length25}
\input{figs/data/VariableLength/Length50}
\input{figs/data/VariableLength/Length100}
\input{figs/data/VariableLength/Length150}

\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{brightgreen}{rgb}{0.616, 0.847, 0.40}
\definecolor{orangehue}{rgb}{1.0,0.627,0.337}
\definecolor{brightblue}{rgb}{0.553, 0.867, 0.8167}



\begin{tikzpicture}
	\begin{axis}[name=rl_obstacle,
	xlabel = {Number of episodes},
	ylabel = {Average Reward},
	ylabel style={yshift=-0.35cm},
	xmin=0,
	xmax=5000,
% 	ymin= 0,
% 	ymax= 1.0,
	label style={font=\small},
	tick label style={font=\small},
	width = 0.45*\textwidth,
	height = 0.25*\textwidth,
	legend cell align={left},
    legend columns=5,
	legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,1.15)}, anchor=north, draw=white!80!black, /tikz/every even column/.append style={column sep=0.01cm}},
	no markers,
	very thick]
    \addplot[red] table[x index={0}, y index={1}] from \shieldvariablelenXIII;
    \addplot[dashed,red] table[x index={0}, y index={1},forget plot] from \noshieldvariablelenXIII;
    \addlegendentry{13}
    \addplot[dashed,blue] table[x index={0}, y index={1},col sep=space,forget plot] from \noshieldvariablelenXXV;
    \addplot[blue] table[x index={0}, y index={1},col sep=space] from \shieldvariablelenXXV;
    \addlegendentry{25}
    \addplot[dashed,brightgreen] table[x index={0}, y index={1},col sep=space,forget plot] from \noshieldvariablelenL;
    \addplot[brightgreen] table[x index={0}, y index={1},col sep=space] from \shieldvariablelenL;
    \addlegendentry{50}
    \addplot[dashed,magenta] table[x index={0}, y index={1},col sep=space,forget plot] from \noshieldvariablelenC;
    \addplot[magenta] table[x index={0}, y index={1},col sep=space] from \shieldvariablelenC;
    \addlegendentry{100}
    \addplot[dashed,orangehue] table[x index={0}, y index={1},col sep=space,forget plot] from \noshieldvariablelenCL;
    \addplot[orangehue] table[x index={0}, y index={1},col sep=space] from \shieldvariablelenCL;
    \addlegendentry{150}
    % \addplot[dashed,green] table[x index={0}, y index={1},col sep=space] from \obstaclenoshieldPPOObs;
    % \addplot[green] table[x index={0}, y index={1},col sep=space] from \obstacleshieldPPOObs;
    % \addplot[dashed,magenta] table[x index={0}, y index={1},col sep=space] from \obstaclenoshieldSACObs;
    % \addplot[magenta] table[x index={0}, y index={1},col sep=space] from \obstacleshieldSACObs;
% 	\input{figs/data/obstacle/noshield_dqn_belief_supp}
% 	\input{figs/data/obstacle/shield_dqn_belief_supp}
	\end{axis}
\end{tikzpicture}


==> var_ep_build.tex <==
\input{figs/data/VariableLength/Length13}
\input{figs/data/VariableLength/Length25}
\input{figs/data/VariableLength/Length50}
\input{figs/data/VariableLength/Length100}
\input{figs/data/VariableLength/Length150}

\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{brightgreen}{rgb}{0.616, 0.847, 0.40}
\definecolor{orangehue}{rgb}{1.0,0.627,0.337}
\definecolor{brightblue}{rgb}{0.553, 0.867, 0.8167}



\begin{tikzpicture}
	\begin{axis}[name=rl_obstacle,
	xlabel = {Number of episodes},
	ylabel = {Average Reward},
	ylabel style={yshift=-0.35cm},
	xmin=0,
	xmax=5000,
% 	ymin= 0,
	ymax= 11.0,
	label style={font=\small},
	tick label style={font=\small},
	width = 0.95*\textwidth,
	height = 0.45*\textwidth,
	legend cell align={left},
    legend columns=5,
	legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.5,1.15)}, anchor=north, draw=white!80!black, /tikz/every even column/.append style={column sep=0.01cm}},
	no markers,
	very thick]
    \addplot[red] table[x index={0}, y index={1}] from \shieldvariablelenXIII;
    \addplot[dashed,red] table[x index={0}, y index={1},forget plot] from \noshieldvariablelenXIII;
    \addlegendentry{13}
    % \addplot[dashed,blue] table[x index={0}, y index={1},col sep=space,forget plot] from \noshieldvariablelenXXV;
    % \addplot[blue] table[x index={0}, y index={1},col sep=space] from \shieldvariablelenXXV;
    % \addlegendentry{25}
    % \addplot[dashed,brightgreen] table[x index={0}, y index={1},col sep=space,forget plot] from \noshieldvariablelenL;
    % \addplot[brightgreen] table[x index={0}, y index={1},col sep=space] from \shieldvariablelenL;
    % \addlegendentry{50}
    % \addplot[dashed,magenta] table[x index={0}, y index={1},col sep=space,forget plot] from \noshieldvariablelenC;
    % \addplot[magenta] table[x index={0}, y index={1},col sep=space] from \shieldvariablelenC;
    % \addlegendentry{100}
    % \addplot[dashed,orangehue] table[x index={0}, y index={1},col sep=space,forget plot] from \noshieldvariablelenCL;
    % \addplot[orangehue] table[x index={0}, y index={1},col sep=space] from \shieldvariablelenCL;
    % \addlegendentry{150}
    % \addplot[dashed,green] table[x index={0}, y index={1},col sep=space] from \obstaclenoshieldPPOObs;
    % \addplot[green] table[x index={0}, y index={1},col sep=space] from \obstacleshieldPPOObs;
    % \addplot[dashed,magenta] table[x index={0}, y index={1},col sep=space] from \obstaclenoshieldSACObs;
    % \addplot[magenta] table[x index={0}, y index={1},col sep=space] from \obstacleshieldSACObs;
% 	\input{figs/data/obstacle/noshield_dqn_belief_supp}
% 	\input{figs/data/obstacle/shield_dqn_belief_supp}
	\end{axis}
\end{tikzpicture}

